Measurement of Inclusive ep Cross Sections at High Q2 at sqrt(s) = 225 and 252 GeV and of the Longitudinal Proton Structure Function FL at HERA

Inclusive ep double differential cross sections for neutral current deep inelastic scattering are measured with the H1 detector at HERA. The data were taken with a lepton beam energy of 27.6 GeV and two proton beam energies of Ep = 460 and 575 GeV corresponding to centre-of-mass energies of 225 and 252 GeV, respectively. The measurements cover the region of 6.5 *10^{-4}<=x<= 0.65 for 35<=Q^2<=800 GeV^2 up to y = 0.85. The measurements are used together with previously published H1 data at Ep = 920 GeV and lower Q2 data at Ep = 460, 575 and 920 GeV to extract the longitudinal proton structure function FL in the region 1.5<=Q^2 <=800 GeV^2.

==> Theory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Neutral and Charged Current Cross Sections}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:theory}



\subsection{Neutral Currents}

The differential cross section for $e^{\pm}p$ scattering after
correction for QED radiative effects can be expressed in terms of
generalised proton structure functions $\tilde{F}$ as
\begin{equation}
\frac{\rm{d}^2\sigma^{\pm}_{\rm NC}}{{\rm d}x{\rm d}Q^2}=
\frac{2\pi\alpha^2}{xQ^4}(Y_+\tilde{F}_2^\pm \mp Y_-x\tilde{F}_3^\pm-y^2\tilde{F}_L^\pm) \cdot (1+\Delta_{\rm NC}^{\rm weak})\,,
\label{eq:ncxsec} 
\end{equation} 
where $Y_{\pm}=1\pm(1-y)^2$ and $y$ characterises the inelasticity of
the interaction. The fine structure constant is defined as
$\alpha\equiv\alpha(Q^2=0)$ and the weak radiative
corrections\footnote{The weak corrections are typically smaller than
  $1\%$ and never more than $3\%$ at the highest $Q^2$ and are not
  applied to the measured cross sections.}  $\Delta_{\rm NC}^{\rm
  weak}$ are defined as in~\cite{hector} in terms of $\alpha$ and the
$Z$ and $W$ boson masses which are taken to be $M_Z=91.187\,{\rm GeV}$ and
$M_W=80.410\,{\rm GeV}$.

The generalised structure functions, $\tilde{F}_{2,3}$, may be
written as linear combinations of the proton structure functions
$F_{2}$, $F_{2,3}^{\gamma Z}$, and $F_{2,3}^{Z}$ containing
information on QCD parton dynamics as well as on the electroweak (EW) 
couplings of the quarks to the neutral vector bosons~\cite{Klein:1983vs}. 
The structure function $F_{2}$ is
associated to pure photon exchange terms, $F_{2,3}^{\gamma Z}$
correspond to photon-$Z$ interference terms and $F_{2,3}^{Z}$ describe
the pure $Z$ exchange terms. In addition the generalised longitudinal
structure function $\tilde{F}_L$ may be similarly decomposed, however
this is an important contribution only at high $y$ and is expected to be negligible at
large $x$ and $Q^2$. The linear combinations for $\tilde{F}_2$ and
$x\tilde{F}_3$ in arbitrarily polarised
$e^{\pm}p$ scattering with lepton polarisation $P_e$ are given by
\begin{eqnarray}
 \tilde{F}^{\pm}_2 = F_2 - (v_e \pm P_e a_e) \kappa  \frac{Q^2}{Q^2+M_Z^2}    F_2^{\gamma Z} 
            + (a_e^2+v_e^2 \pm P_e 2v_e a_e) \kappa^2 \left[\frac{Q^2}{Q^2+M_Z^2}\right]^2 F_2^Z \,,
\label{eq:F2}\\
 x\tilde{F}^{\pm}_3 = -(a_e \pm P_e v_e)   \kappa    \frac{Q^2}{Q^2+M_Z^2}    xF_3^{\gamma Z} 
       + (2a_ev_e \pm P_e [v_e^2 + a_e^2] ) \kappa^2 \left[\frac{Q^2}{Q^2+M_Z^2}\right]^2 xF_3^Z\,,
\label{eq:F3}
\end{eqnarray}
with $\kappa^{-1}=4\frac{M_W^2}{M_Z^2}(1-\frac{M_W^2}{M_Z^2})$
in the on-mass-shell scheme. The quantities $v_e$ and $a_e$ are the
vector and axial-vector couplings of the electron to the $Z$ boson. 

It can be seen from equations\,\ref{eq:F2} and \ref{eq:F3} that different
combinations of structure functions may be experimentally
determined
by scattering longitudinally polarised leptons on unpolarised protons.
In particular, since $v_e$ is small, a
measurement of the polarisation asymmetry for fixed lepton charge
allows the parity violating structure function $F_2^{\gamma Z}$ to be
measured.

In the quark-parton model (QPM), the hadronic structure functions are
related to linear combinations of sums and differences of the quark
and anti-quark momentum distributions $xq(x,Q^2)$ and
$x\bar{q}(x,Q^2)$. The structure function $\tilde{F}_2$ is
determined by the sum of quarks and anti-quark momentum distributions,
whereas the structure function $x\tilde{F}_3$ is
determined by the difference of quarks and anti-quark momentum
distributions and is therefore sensitive to the valence quark
distributions:
\begin{eqnarray}
  \left[F_2,F_2^{\gamma Z},F_2^Z\right] &=& x\sum_q [e_q^2,2e_qv_q,v_q^2+a_q^2](q+\bar{q})\,, \\
  \left[xF_3^{\gamma Z},xF_3^Z \right] &=& 2x \sum_q[e_qa_q,v_qa_q](q-\bar{q})\,.
\label{eq:SF2} 
\end{eqnarray} 
Here $v_q$ and $a_q$ are the vector and axial-vector couplings of the
quarks to the $Z$ boson and $e_q$ is the charge of the quark of flavour $q$.

The reduced NC cross section is defined by
\begin{equation}
\tilde{\sigma}_{\rm NC}^{\pm}(x,Q^2)\equiv
\frac{\rm{d}^2\sigma^{\pm}_{\rm NC}}{{\rm d}x{\rm d}Q^2}\frac{xQ^4}{2\pi\alpha^2}\frac{1}{Y_+}\equiv
\left( \tilde{F}_2^\pm \mp \frac{Y_-}{Y_+}x\tilde{F}_3^\pm-\frac{y^2}{Y_+}\tilde{F}_L^\pm \right) (1+\Delta_{\rm NC}^{\rm weak})\,.
\label{eq:Rnc}
\end{equation} 

%%%%%%%%%%%%%%%%%%%%%%

\subsection{Charged Currents}

The differential CC cross section for $e^{\pm}p$
scattering of polarised leptons with unpolarised protons, corrected
for QED radiative effects, can be expressed as
\begin{equation}
\frac{{\rm d}^2\sigma^{\pm}_{\rm CC}}{{\rm d}x {\rm d}\QQ} = (1\pm P_e)
 \frac{G_F^2}{4\pi x } \left[\frac{M_W^2}{M_W^2+Q^2} \right]^2 
\left(Y_+ W^{\pm}_2 \mp Y_{-}xW^{\pm}_3 -y^2W^{\pm}_L \right ) \cdot (1+\Delta_{\rm CC}^{\rm weak})\,,
\label{eq:ccxsec}
\end{equation}
 
where $G_F$ is the Fermi constant defined using the weak boson
masses~\cite{hector}. Here $W^{\pm}_2$, $xW^{\pm}_3$ and $W^{\pm}_L$
are the structure functions for CC $e^{\pm}p$ scattering, and
$\Delta^{\rm CC}_{\rm weak}$ represents the weak radiative corrections
for CC interactions.
% which is not applied to the measured cross sections. 
From equation\,\ref{eq:ccxsec} it can be seen that the
cross section has a linear dependence on the polarisation of the
electron beam $P_e$. For a fully right handed $e^-$ beam ($P_e=1$),
or a fully left handed $e^+$ beam ($P_e=-1$) the cross section is
identically zero in the Standard Model (SM). In the QPM $W^{\pm}_L\equiv 0$, and the
structure functions $W^{\pm}_2$ and $xW^{\pm}_3$ are expressed as the
flavour dependent sum and difference of the quark and anti-quark
momentum distributions. In the CC case only the positively charged
quarks contribute to $W^-$ mediated scattering and conversely only
negatively charged quarks couple to the exchanged $W^+$ boson, thus
\begin{eqnarray}
W^-_2 \! &=&\! x(U+\overline{D})\,,\hspace{5.5mm} W^+_2 = x(\overline{U}+ D )\,,\\ 
xW^-_3 \!&=&\! x(U-\overline{D})\,,\hspace{3mm} xW^+_3 = x(D -\overline{U})\,,
\end{eqnarray}
where, below the $b$ quark mass threshold
%\begin{eqnarray}
\begin{equation}
\label{eq:ud}
 U = u + c\,,~~ %  \nonumber\\
\overline{U}= \bu + \bc\,,~~% \nonumber\\
 D = d + s\,, ~~ %\nonumber\\
\overline{D}= \bd + \bs\,, 
%\end{eqnarray}
\end{equation}
where $u$, $d$, $s$, $c$ represent quark densities of each flavour in
the standard notation.  Here $U$ represents the sum of up-type, and
$D$ the sum of down-type quark densities.

The reduced CC cross section is then defined as
\begin{equation}
\label{eq:Rcc}
\tilde{\sigma}_{\rm CC}(x,Q^2) \equiv  
\frac{4 \pi  x}{ G_F^2}
\left[ \frac {M_W^2+Q^2} {M_W^2} \right]^2
          \frac{{\rm d}^2 \sigma_{\rm CC}}{{\rm d}x{\rm d}Q^2}\,\,.
\end{equation}


==> plots/ave_fl-allq2.tex <==
$   1.5 $ &$ 0.279 \times 10^{-4}$ & $ 0.087 $ &$ 0.113 $ &$ 0.186 $ &$ 0.053 $ &$0.224$  \\
$    2. $ &$ 0.427 \times 10^{-4}$ & $ 0.127 $ &$ 0.039 $ &$ 0.074 $ &$ 0.044 $ &$0.095$  \\
$   2.5 $ &$ 0.588 \times 10^{-4}$ & $ 0.155 $ &$ 0.025 $ &$ 0.050 $ &$ 0.053 $ &$0.077$  \\
$   3.5 $ &$ 0.877 \times 10^{-4}$ & $ 0.226 $ &$ 0.021 $ &$ 0.049 $ &$ 0.040 $ &$0.067$  \\
$    5. $ &$ 0.129 \times 10^{-3}$ & $ 0.313 $ &$ 0.022 $ &$ 0.055 $ &$ 0.045 $ &$0.074$  \\
$   6.5 $ &$ 0.169 \times 10^{-3}$ & $ 0.263 $ &$ 0.023 $ &$ 0.058 $ &$ 0.050 $ &$0.080$  \\
$   8.5 $ &$ 0.224 \times 10^{-3}$ & $ 0.214 $ &$ 0.025 $ &$ 0.062 $ &$ 0.051 $ &$0.084$  \\
$   12. $ &$ 0.319 \times 10^{-3}$ & $ 0.325 $ &$ 0.026 $ &$ 0.051 $ &$ 0.044 $ &$0.072$  \\
$   15. $ &$ 0.402 \times 10^{-3}$ & $ 0.267 $ &$ 0.027 $ &$ 0.051 $ &$ 0.042 $ &$0.071$  \\
$   20. $ &$ 0.540 \times 10^{-3}$ & $ 0.328 $ &$ 0.029 $ &$ 0.053 $ &$ 0.040 $ &$0.072$  \\
$   25. $ &$ 0.687 \times 10^{-3}$ & $ 0.283 $ &$ 0.029 $ &$ 0.061 $ &$ 0.037 $ &$0.077$  \\
$   35. $ &$ 0.995 \times 10^{-3}$ & $ 0.191 $ &$ 0.038 $ &$ 0.064 $ &$ 0.040 $ &$0.085$  \\
$   45. $ &$ 0.124 \times 10^{-2}$ & $ 0.279 $ &$ 0.045 $ &$ 0.065 $ &$ 0.045 $ &$0.091$  \\
$   60. $ &$ 0.159 \times 10^{-2}$ & $ 0.285 $ &$ 0.053 $ &$ 0.064 $ &$ 0.042 $ &$0.093$  \\
$   90. $ &$ 0.245 \times 10^{-2}$ & $ 0.086 $ &$ 0.063 $ &$ 0.063 $ &$ 0.037 $ &$0.097$  \\
$  120. $ &$ 0.306 \times 10^{-2}$ & $ 0.186 $ &$ 0.054 $ &$ 0.080 $ &$ 0.023 $ &$0.100$  \\
$  150. $ &$ 0.404 \times 10^{-2}$ & $ 0.218 $ &$ 0.044 $ &$ 0.068 $ &$ 0.031 $ &$0.087$  \\
$  200. $ &$ 0.541 \times 10^{-2}$ & $ 0.089 $ &$ 0.055 $ &$ 0.073 $ &$ 0.028 $ &$0.095$  \\
$  250. $ &$ 0.754 \times 10^{-2}$ & $ 0.159 $ &$ 0.064 $ &$ 0.075 $ &$ 0.029 $ &$0.103$  \\
$  300. $ &$ 0.845 \times 10^{-2}$ & $ 0.202 $ &$ 0.077 $ &$ 0.080 $ &$ 0.026 $ &$0.114$  \\
$  400. $ &$ 0.111 \times 10^{-1}$ & $ -.127 $ &$ 0.084 $ &$ 0.074 $ &$ 0.022 $ &$0.114$  \\
$  500. $ &$ 0.142 \times 10^{-1}$ & $ -.008 $ &$ 0.103 $ &$ 0.071 $ &$ 0.020 $ &$0.126$  \\
$  650. $ &$ 0.187 \times 10^{-1}$ & $ 0.045 $ &$ 0.113 $ &$ 0.074 $ &$ 0.019 $ &$0.136$  \\
$  800. $ &$ 0.231 \times 10^{-1}$ & $ 0.278 $ &$ 0.119 $ &$ 0.079 $ &$ 0.018 $ &$0.144$  \\


==> plots/ave_fl.tex <==
$   1.5 $ &$ 0.279 \times 10^{-4}$ & $ 0.088 $ &$ 0.113 $ &$ 0.186 $ &$ 0.053 $ &$0.224$  \\
$    2. $ &$ 0.427 \times 10^{-4}$ & $ 0.127 $ &$ 0.039 $ &$ 0.074 $ &$ 0.044 $ &$0.095$  \\
$   2.5 $ &$ 0.588 \times 10^{-4}$ & $ 0.156 $ &$ 0.025 $ &$ 0.050 $ &$ 0.053 $ &$0.077$  \\
$   3.5 $ &$ 0.877 \times 10^{-4}$ & $ 0.227 $ &$ 0.021 $ &$ 0.049 $ &$ 0.040 $ &$0.067$  \\
$    5. $ &$ 0.129 \times 10^{-3}$ & $ 0.314 $ &$ 0.022 $ &$ 0.055 $ &$ 0.045 $ &$0.074$  \\
$   6.5 $ &$ 0.169 \times 10^{-3}$ & $ 0.264 $ &$ 0.023 $ &$ 0.058 $ &$ 0.050 $ &$0.080$  \\
$   8.5 $ &$ 0.224 \times 10^{-3}$ & $ 0.216 $ &$ 0.025 $ &$ 0.062 $ &$ 0.051 $ &$0.084$  \\
$   12. $ &$ 0.319 \times 10^{-3}$ & $ 0.324 $ &$ 0.026 $ &$ 0.051 $ &$ 0.044 $ &$0.072$  \\
$   15. $ &$ 0.402 \times 10^{-3}$ & $ 0.266 $ &$ 0.027 $ &$ 0.051 $ &$ 0.042 $ &$0.071$  \\
$   20. $ &$ 0.540 \times 10^{-3}$ & $ 0.327 $ &$ 0.029 $ &$ 0.053 $ &$ 0.040 $ &$0.072$  \\
$   25. $ &$ 0.687 \times 10^{-3}$ & $ 0.282 $ &$ 0.029 $ &$ 0.061 $ &$ 0.037 $ &$0.077$  \\
$   35. $ &$ 0.958 \times 10^{-3}$ & $ 0.213 $ &$ 0.035 $ &$ 0.059 $ &$ 0.040 $ &$0.080$  \\
$   45. $ &$ 0.121 \times 10^{-2}$ & $ 0.303 $ &$ 0.043 $ &$ 0.060 $ &$ 0.044 $ &$0.086$  \\
$   60. $ &$ 0.157 \times 10^{-2}$ & $ 0.315 $ &$ 0.051 $ &$ 0.060 $ &$ 0.044 $ &$0.090$  \\
$   90. $ &$ 0.243 \times 10^{-2}$ & $ 0.125 $ &$ 0.061 $ &$ 0.062 $ &$ 0.039 $ &$0.095$  \\
$  120. $ &$ 0.303 \times 10^{-2}$ & $ 0.198 $ &$ 0.054 $ &$ 0.077 $ &$ 0.029 $ &$0.098$  \\
$  150. $ &$ 0.402 \times 10^{-2}$ & $ 0.264 $ &$ 0.044 $ &$ 0.068 $ &$ 0.035 $ &$0.088$  \\
$  200. $ &$ 0.541 \times 10^{-2}$ & $ 0.150 $ &$ 0.056 $ &$ 0.073 $ &$ 0.034 $ &$0.099$  \\
$  250. $ &$ 0.736 \times 10^{-2}$ & $ 0.196 $ &$ 0.061 $ &$ 0.075 $ &$ 0.033 $ &$0.102$  \\
$  346. $ &$ 0.986 \times 10^{-2}$ & $ 0.039 $ &$ 0.059 $ &$ 0.057 $ &$ 0.029 $ &$0.087$  \\
$  636. $ &$ 0.184 \times 10^{-1}$ & $ 0.152 $ &$ 0.066 $ &$ 0.045 $ &$ 0.020 $ &$0.082$  \\


==> plots/correlation.tex <==
\begin{table}
%\renewcommand{\arraystretch}{1.22} % increase space between table rows\begin{table}[htp]
\begin{center}
\begin{tabular}{l|cccccccc}
\hline
 Data set & \multicolumn{2}{c}{$\delta^{\cal L}$} &   $\delta^E$ & $\delta^{\theta}$ &  $\delta^h$
 &$\delta^N$&
$\delta^B$&$\delta^S$ \\ \hline 
$e^+$ Combined low $Q^2$ & $\delta^{{\cal L}1} $ &&&&&&& \\ \hline 
$e^+$ Combined low $E_p$ & $\delta^{{\cal L}1} $ &&&&&&& \\ \hline
$e^+$ NC $94$-$97$ & $\delta^{{\cal L}1}$ & $\delta^{{\cal L}2}$ & $\delta^{E1}$ &$\delta^{\theta1}$ & $\delta^{h1}$ & $\delta^{N1}$ & $\delta^{B1}$ & $-$ \\
$e^-$ NC $98$-$99$ & $\delta^{{\cal L}1}$ & $\delta^{{\cal L}3}$ & $\delta^{E1}$ &$\delta^{\theta2}$ & $\delta^{h1}$ & $\delta^{N1}$ & $\delta^{B1}$ & $-$ \\
$e^-$ NC $98$-$99$ {\em high $y$} &  $\delta^{{\cal L}1}$ & $\delta^{{\cal L}3}$ & $\delta^{E1}$  & $\delta^{\theta 2}$ & $\delta^{h1}$ & $\delta^{N1}$ & $-$ & $\delta^{S1}$\\
$e^+$ NC $99$-$00$ &  $\delta^{{\cal L}1}$ & $\delta^{{\cal L}4}$ & $\delta^{E1}$  & $\delta^{\theta 2}$ & $\delta^{h1}$ & $\delta^{N1}$ & $\delta^{B1}$ & $\delta^{S1}$\\
$e^+$ NC {\em high $y$}   & $\delta^{{\cal L}5}$ & $\delta^{{\cal L}6}, \delta^{{\cal L}7}$ & $\delta^{E2}$ &$\delta^{\theta3}$ & $\delta^{h2}$ & $\delta^{N2}$ &$-$ & $\delta^{S2}$\\
$e^-$ NC {\em high $y$}   & $\delta^{{\cal L}5}$ & $\delta^{{\cal L}8}, \delta^{{\cal L}9}$ & $\delta^{E2}$ &$\delta^{\theta3}$ & $\delta^{h2}$ & $\delta^{N2}$ & $-$ & $\delta^{S2}$\\
$e^+$ NC $920$  & $\delta^{{\cal L}5}$ & $\delta^{{\cal L}6}$ & $\delta^{E2}$ &$\delta^{\theta3}$ & $\delta^{h2}$ & $\delta^{N2}$ & $\delta^{B1}$ &  $-$ \\
$e^+$ NC $460$  & $\delta^{{\cal L}5}$ & $\delta^{{\cal L}7}$ & $\delta^{E2}$ &$\delta^{\theta3}$ & $\delta^{h2}$ & $\delta^{N2}$ & $\delta^{B1}$ &  $-$ \\
$e^-$ NC $575$  & $\delta^{{\cal L}5}$ & $\delta^{{\cal L}8}$ & $\delta^{E2}$ &$\delta^{\theta3}$ & $\delta^{h2}$ & $\delta^{N2}$ & $\delta^{B1}$ &  $-$ \\
\hline
\end{tabular}        
\end{center}
\caption 
 { Correlation of systematic error sources across different data
   sets. For each of the nine correlated systematic error sources one
   or more parameters are included in the fit procedure. The sources
   considered are due to the luminosity uncertainty
   ($\delta^{\mathcal{L}}$), the electron energy uncertainty
   ($\delta^E$), the electron polar angle measurement
   ($\delta^{\theta}$), the hadronic energy uncertainty
   ($\delta^{h}$), the uncertainty due to noise subtraction
   ($\delta^{N}$), and the error of the background charge asymmetry
   ($\delta^{S}$).  The table entries indicate the correlation of the
   error sources across the data sets where each numerical index
   corresponds to a fit parameter for the given error source. For
   example, the uncertainty due to the noise subtraction is the same
   for all data sets in HERA\,I leading to one common parameter in the
   fit ($\delta^{N1}$)}
\label{tab:correlation}
\end{table}
%\renewcommand{\arraystretch}{1.00} % set table row spacing back to default


==> plots/flf2615.tex <==
\begin{table}[htbp] 
\begin{center} 
\tiny 
\begin{tabular}{|r|c|c|r|r|r|r|r|r|r|r|r|r|} 
\hline 
$Q^2$ & $x$ &
$F_{L}$ &
$\Delta_{\rm stat}F_{L}$ &
$\Delta_{\rm uncor}F_{L}$ &
$\Delta_{\rm cor}F_{L}$ &
$\Delta_{\rm tot}F_{L}$ &
$F_{2}$ &
$\Delta_{\rm stat}F_{2}$ &
$\Delta_{\rm uncor}F_{2}$ &
$\Delta_{\rm cor}F_{2}$ &
$\Delta_{\rm tot}F_{2}$ &
$\rho$ \\ 
(GeV$^2$) & & & & & & & & & & & & \\
\hline
$   1.5 $&$    0.279 \times 10^{-4} $&$ 0.088 $&$ 0.113 $&$ 0.186 $&$ 0.053 $&$ 0.224 $&$ 0.732 $&$ 0.066 $&$ 0.096 $&$ 0.028 $&$ 0.120 $&$ 0.882$\\
$    2. $&$    0.372 \times 10^{-4} $&$ 0.110 $&$ 0.069 $&$ 0.131 $&$ 0.062 $&$ 0.160 $&$ 0.843 $&$ 0.028 $&$ 0.051 $&$ 0.032 $&$ 0.066 $&$ 0.855$\\
$    2. $&$    0.415 \times 10^{-4} $&$ 0.437 $&$ 0.110 $&$ 0.181 $&$ 0.071 $&$ 0.223 $&$ 0.904 $&$ 0.039 $&$ 0.060 $&$ 0.030 $&$ 0.078 $&$ 0.852$\\
$    2. $&$    0.464 \times 10^{-4} $&$ 0.043 $&$ 0.052 $&$ 0.104 $&$ 0.033 $&$ 0.121 $&$ 0.740 $&$ 0.033 $&$ 0.052 $&$ 0.009 $&$ 0.062 $&$ 0.822$\\
$   2.5 $&$    0.465 \times 10^{-4} $&$ 0.013 $&$ 0.057 $&$ 0.120 $&$ 0.046 $&$ 0.141 $&$ 0.846 $&$ 0.022 $&$ 0.045 $&$ 0.016 $&$ 0.053 $&$ 0.856$\\
$   2.5 $&$    0.519 \times 10^{-4} $&$ 0.103 $&$ 0.062 $&$ 0.129 $&$ 0.042 $&$ 0.149 $&$ 0.897 $&$ 0.023 $&$ 0.045 $&$ 0.016 $&$ 0.053 $&$ 0.860$\\
$   2.5 $&$    0.580 \times 10^{-4} $&$ 0.174 $&$ 0.047 $&$ 0.090 $&$ 0.058 $&$ 0.117 $&$ 0.889 $&$ 0.021 $&$ 0.034 $&$ 0.028 $&$ 0.049 $&$ 0.821$\\
$   2.5 $&$    0.658 \times 10^{-4} $&$ 0.169 $&$ 0.043 $&$ 0.099 $&$ 0.063 $&$ 0.125 $&$ 0.865 $&$ 0.019 $&$ 0.035 $&$ 0.031 $&$ 0.050 $&$ 0.840$\\
$   2.5 $&$    0.759 \times 10^{-4} $&$ 0.413 $&$ 0.096 $&$ 0.155 $&$ 0.079 $&$ 0.198 $&$ 0.877 $&$ 0.024 $&$ 0.035 $&$ 0.026 $&$ 0.050 $&$ 0.783$\\
$   3.5 $&$    0.651 \times 10^{-4} $&$ 0.130 $&$ 0.065 $&$ 0.135 $&$ 0.052 $&$ 0.158 $&$ 0.973 $&$ 0.025 $&$ 0.050 $&$ 0.022 $&$ 0.060 $&$ 0.846$\\
$   3.5 $&$    0.727 \times 10^{-4} $&$ 0.199 $&$ 0.061 $&$ 0.133 $&$ 0.044 $&$ 0.152 $&$ 0.989 $&$ 0.024 $&$ 0.047 $&$ 0.021 $&$ 0.057 $&$ 0.850$\\
$   3.5 $&$    0.812 \times 10^{-4} $&$ 0.253 $&$ 0.044 $&$ 0.094 $&$ 0.041 $&$ 0.112 $&$ 0.981 $&$ 0.019 $&$ 0.036 $&$ 0.016 $&$ 0.044 $&$ 0.811$\\
$   3.5 $&$    0.921 \times 10^{-4} $&$ 0.230 $&$ 0.037 $&$ 0.099 $&$ 0.037 $&$ 0.112 $&$ 0.968 $&$ 0.015 $&$ 0.033 $&$ 0.014 $&$ 0.039 $&$ 0.816$\\
$   3.5 $&$    0.106 \times 10^{-3} $&$ 0.155 $&$ 0.049 $&$ 0.123 $&$ 0.046 $&$ 0.141 $&$ 0.934 $&$ 0.015 $&$ 0.032 $&$ 0.010 $&$ 0.037 $&$ 0.797$\\
$   3.5 $&$    0.141 \times 10^{-3} $&$ 0.665 $&$ 0.112 $&$ 0.221 $&$ 0.123 $&$ 0.276 $&$ 0.937 $&$ 0.011 $&$ 0.028 $&$ 0.012 $&$ 0.032 $&$ 0.735$\\
$    5. $&$    0.931 \times 10^{-4} $&$ 0.411 $&$ 0.081 $&$ 0.162 $&$ 0.068 $&$ 0.193 $&$ 1.149 $&$ 0.031 $&$ 0.060 $&$ 0.031 $&$ 0.075 $&$ 0.846$\\
$    5. $&$    0.104 \times 10^{-3} $&$ 0.344 $&$ 0.065 $&$ 0.142 $&$ 0.044 $&$ 0.163 $&$ 1.072 $&$ 0.027 $&$ 0.052 $&$ 0.024 $&$ 0.063 $&$ 0.859$\\
$    5. $&$    0.116 \times 10^{-3} $&$ 0.258 $&$ 0.048 $&$ 0.108 $&$ 0.049 $&$ 0.128 $&$ 1.127 $&$ 0.021 $&$ 0.042 $&$ 0.018 $&$ 0.050 $&$ 0.828$\\
$    5. $&$    0.131 \times 10^{-3} $&$ 0.306 $&$ 0.037 $&$ 0.109 $&$ 0.041 $&$ 0.122 $&$ 1.082 $&$ 0.016 $&$ 0.037 $&$ 0.017 $&$ 0.044 $&$ 0.830$\\
$    5. $&$    0.152 \times 10^{-3} $&$ 0.224 $&$ 0.044 $&$ 0.134 $&$ 0.045 $&$ 0.148 $&$ 1.060 $&$ 0.014 $&$ 0.034 $&$ 0.015 $&$ 0.040 $&$ 0.834$\\
$    5. $&$    0.201 \times 10^{-3} $&$ 0.533 $&$ 0.057 $&$ 0.203 $&$ 0.084 $&$ 0.227 $&$ 1.018 $&$ 0.008 $&$ 0.028 $&$ 0.012 $&$ 0.032 $&$ 0.809$\\
$   6.5 $&$    0.121 \times 10^{-3} $&$ 0.435 $&$ 0.096 $&$ 0.179 $&$ 0.077 $&$ 0.218 $&$ 1.215 $&$ 0.037 $&$ 0.066 $&$ 0.027 $&$ 0.080 $&$ 0.853$\\
$   6.5 $&$    0.135 \times 10^{-3} $&$ 0.199 $&$ 0.071 $&$ 0.151 $&$ 0.042 $&$ 0.172 $&$ 1.103 $&$ 0.030 $&$ 0.055 $&$ 0.020 $&$ 0.066 $&$ 0.862$\\
$   6.5 $&$    0.151 \times 10^{-3} $&$ 0.137 $&$ 0.051 $&$ 0.114 $&$ 0.054 $&$ 0.136 $&$ 1.135 $&$ 0.023 $&$ 0.044 $&$ 0.023 $&$ 0.055 $&$ 0.844$\\
$   6.5 $&$    0.171 \times 10^{-3} $&$ 0.357 $&$ 0.040 $&$ 0.119 $&$ 0.044 $&$ 0.133 $&$ 1.158 $&$ 0.017 $&$ 0.041 $&$ 0.020 $&$ 0.048 $&$ 0.844$\\
$   6.5 $&$    0.197 \times 10^{-3} $&$ 0.318 $&$ 0.044 $&$ 0.145 $&$ 0.053 $&$ 0.161 $&$ 1.147 $&$ 0.014 $&$ 0.038 $&$ 0.019 $&$ 0.044 $&$ 0.855$\\
$   6.5 $&$    0.262 \times 10^{-3} $&$ 0.188 $&$ 0.046 $&$ 0.205 $&$ 0.090 $&$ 0.229 $&$ 1.044 $&$ 0.007 $&$ 0.029 $&$ 0.017 $&$ 0.034 $&$ 0.842$\\
$   8.5 $&$    0.158 \times 10^{-3} $&$ 0.499 $&$ 0.109 $&$ 0.195 $&$ 0.095 $&$ 0.243 $&$ 1.352 $&$ 0.044 $&$ 0.074 $&$ 0.033 $&$ 0.092 $&$ 0.845$\\
$   8.5 $&$    0.177 \times 10^{-3} $&$ 0.489 $&$ 0.089 $&$ 0.184 $&$ 0.051 $&$ 0.210 $&$ 1.335 $&$ 0.038 $&$ 0.067 $&$ 0.022 $&$ 0.080 $&$ 0.862$\\
$   8.5 $&$    0.197 \times 10^{-3} $&$ 0.271 $&$ 0.057 $&$ 0.123 $&$ 0.058 $&$ 0.147 $&$ 1.196 $&$ 0.027 $&$ 0.048 $&$ 0.021 $&$ 0.059 $&$ 0.841$\\
$   8.5 $&$    0.224 \times 10^{-3} $&$ 0.242 $&$ 0.045 $&$ 0.125 $&$ 0.042 $&$ 0.139 $&$ 1.158 $&$ 0.019 $&$ 0.043 $&$ 0.017 $&$ 0.050 $&$ 0.849$\\
$   8.5 $&$    0.258 \times 10^{-3} $&$-0.123 $&$ 0.045 $&$ 0.140 $&$ 0.051 $&$ 0.156 $&$ 1.038 $&$ 0.015 $&$ 0.036 $&$ 0.016 $&$ 0.042 $&$ 0.853$\\
$   8.5 $&$    0.342 \times 10^{-3} $&$ 0.167 $&$ 0.045 $&$ 0.216 $&$ 0.089 $&$ 0.238 $&$ 1.095 $&$ 0.007 $&$ 0.030 $&$ 0.017 $&$ 0.035 $&$ 0.846$\\
$   12. $&$    0.223 \times 10^{-3} $&$ 0.094 $&$ 0.101 $&$ 0.159 $&$ 0.084 $&$ 0.206 $&$ 1.314 $&$ 0.039 $&$ 0.041 $&$ 0.044 $&$ 0.072 $&$ 0.855$\\
$   12. $&$    0.249 \times 10^{-3} $&$ 0.544 $&$ 0.098 $&$ 0.155 $&$ 0.058 $&$ 0.193 $&$ 1.389 $&$ 0.035 $&$ 0.035 $&$ 0.028 $&$ 0.057 $&$ 0.835$\\
$   12. $&$    0.278 \times 10^{-3} $&$ 0.281 $&$ 0.059 $&$ 0.098 $&$ 0.047 $&$ 0.124 $&$ 1.310 $&$ 0.024 $&$ 0.024 $&$ 0.019 $&$ 0.039 $&$ 0.757$\\
$   12. $&$    0.316 \times 10^{-3} $&$ 0.248 $&$ 0.050 $&$ 0.100 $&$ 0.038 $&$ 0.118 $&$ 1.258 $&$ 0.019 $&$ 0.022 $&$ 0.015 $&$ 0.033 $&$ 0.733$\\
$   12. $&$    0.364 \times 10^{-3} $&$ 0.435 $&$ 0.055 $&$ 0.121 $&$ 0.041 $&$ 0.139 $&$ 1.268 $&$ 0.016 $&$ 0.022 $&$ 0.013 $&$ 0.030 $&$ 0.728$\\
$   12. $&$    0.483 \times 10^{-3} $&$ 0.414 $&$ 0.050 $&$ 0.162 $&$ 0.064 $&$ 0.181 $&$ 1.189 $&$ 0.007 $&$ 0.016 $&$ 0.012 $&$ 0.021 $&$ 0.651$\\
$   15. $&$    0.279 \times 10^{-3} $&$ 0.510 $&$ 0.109 $&$ 0.183 $&$ 0.085 $&$ 0.230 $&$ 1.485 $&$ 0.040 $&$ 0.047 $&$ 0.049 $&$ 0.079 $&$ 0.854$\\
$   15. $&$    0.312 \times 10^{-3} $&$ 0.148 $&$ 0.088 $&$ 0.150 $&$ 0.052 $&$ 0.181 $&$ 1.370 $&$ 0.032 $&$ 0.035 $&$ 0.027 $&$ 0.054 $&$ 0.834$\\
$   15. $&$    0.348 \times 10^{-3} $&$ 0.188 $&$ 0.061 $&$ 0.099 $&$ 0.039 $&$ 0.122 $&$ 1.329 $&$ 0.023 $&$ 0.023 $&$ 0.017 $&$ 0.036 $&$ 0.748$\\
$   15. $&$    0.395 \times 10^{-3} $&$ 0.419 $&$ 0.051 $&$ 0.100 $&$ 0.036 $&$ 0.118 $&$ 1.321 $&$ 0.017 $&$ 0.021 $&$ 0.015 $&$ 0.031 $&$ 0.710$\\
$   15. $&$    0.455 \times 10^{-3} $&$ 0.257 $&$ 0.062 $&$ 0.117 $&$ 0.045 $&$ 0.140 $&$ 1.269 $&$ 0.015 $&$ 0.018 $&$ 0.013 $&$ 0.027 $&$ 0.693$\\
$   15. $&$    0.604 \times 10^{-3} $&$ 0.066 $&$ 0.054 $&$ 0.157 $&$ 0.066 $&$ 0.179 $&$ 1.180 $&$ 0.007 $&$ 0.014 $&$ 0.012 $&$ 0.019 $&$ 0.620$\\
$   20. $&$    0.372 \times 10^{-3} $&$ 0.216 $&$ 0.116 $&$ 0.197 $&$ 0.065 $&$ 0.238 $&$ 1.452 $&$ 0.041 $&$ 0.051 $&$ 0.033 $&$ 0.073 $&$ 0.877$\\
$   20. $&$    0.415 \times 10^{-3} $&$ 0.322 $&$ 0.092 $&$ 0.158 $&$ 0.044 $&$ 0.188 $&$ 1.424 $&$ 0.032 $&$ 0.037 $&$ 0.021 $&$ 0.054 $&$ 0.837$\\
$   20. $&$    0.464 \times 10^{-3} $&$ 0.412 $&$ 0.070 $&$ 0.108 $&$ 0.037 $&$ 0.134 $&$ 1.396 $&$ 0.024 $&$ 0.025 $&$ 0.015 $&$ 0.037 $&$ 0.752$\\
$   20. $&$    0.526 \times 10^{-3} $&$ 0.358 $&$ 0.052 $&$ 0.103 $&$ 0.037 $&$ 0.121 $&$ 1.354 $&$ 0.018 $&$ 0.021 $&$ 0.015 $&$ 0.032 $&$ 0.708$\\
$   20. $&$    0.607 \times 10^{-3} $&$ 0.304 $&$ 0.062 $&$ 0.119 $&$ 0.041 $&$ 0.140 $&$ 1.295 $&$ 0.015 $&$ 0.019 $&$ 0.013 $&$ 0.027 $&$ 0.693$\\
$   20. $&$    0.805 \times 10^{-3} $&$ 0.212 $&$ 0.060 $&$ 0.163 $&$ 0.068 $&$ 0.186 $&$ 1.222 $&$ 0.007 $&$ 0.014 $&$ 0.012 $&$ 0.019 $&$ 0.608$\\
$   25. $&$    0.493 \times 10^{-3} $&$ 0.363 $&$ 0.072 $&$ 0.157 $&$ 0.043 $&$ 0.178 $&$ 1.484 $&$ 0.022 $&$ 0.040 $&$ 0.024 $&$ 0.052 $&$ 0.851$\\
$   25. $&$    0.616 \times 10^{-3} $&$ 0.284 $&$ 0.043 $&$ 0.089 $&$ 0.031 $&$ 0.103 $&$ 1.382 $&$ 0.013 $&$ 0.021 $&$ 0.014 $&$ 0.028 $&$ 0.698$\\
$   25. $&$    0.759 \times 10^{-3} $&$ 0.296 $&$ 0.065 $&$ 0.124 $&$ 0.042 $&$ 0.146 $&$ 1.330 $&$ 0.015 $&$ 0.020 $&$ 0.013 $&$ 0.028 $&$ 0.700$\\
$   25. $&$    0.101 \times 10^{-2} $&$ 0.168 $&$ 0.064 $&$ 0.167 $&$ 0.068 $&$ 0.191 $&$ 1.236 $&$ 0.007 $&$ 0.014 $&$ 0.012 $&$ 0.020 $&$ 0.616$\\
\hline 
\end{tabular} 
\end{center} 
%\captcont{
\caption{
   \label{tab:flf2a} The proton structure functions $F_L$ and
   $F_2$ measured at the given values of $Q^2$ and $x$ without model
   assumptions.  $\Delta_{\rm stat}F_{L}$, $\Delta_{\rm uncor}F_{L}$,
   $\Delta_{\rm cor}F_{L}$ and $\Delta_{\rm tot}F_{L}$ are the
   statistical, uncorrelated systematic, correlated systematic, and
   total uncertainty on $F_L$ respectively.  $\Delta_{\rm stat}F_{2}$,
   $\Delta_{\rm uncor}F_{2}$, $\Delta_{\rm cor}F_{2}$ and $\Delta_{\rm
     tot}F_{2}$ are the statistical, uncorrelated systematic and total
   uncertainty on $F_2$, respectively.  $\rho$ is the correlation
   coefficient between the $F_L$ and $F_2$ values.}

\end{table} 


\begin{table}[htbp] 
\begin{center} 
\tiny 
\begin{tabular}{|r|c|c|r|r|r|r|r|r|r|r|r|r|} 
\hline 
$Q^2$ & $x$ &
$F_{L}$ &
$\Delta_{\rm stat}F_{L}$ &
$\Delta_{\rm uncor}F_{L}$ &
$\Delta_{\rm cor}F_{L}$ &
$\Delta_{\rm tot}F_{L}$ &
$F_{2}$ &
$\Delta_{\rm stat}F_{2}$ &
$\Delta_{\rm uncor}F_{2}$ &
$\Delta_{\rm cor}F_{2}$ &
$\Delta_{\rm tot}F_{2}$ &
$\rho$ \\ 
(GeV$^2$) & & & & & & & & & & & & \\
\hline
$   35. $&$    0.651 \times 10^{-3} $&$ 0.453 $&$ 0.124 $&$ 0.214 $&$ 0.091 $&$ 0.264 $&$ 1.612 $&$ 0.043 $&$ 0.058 $&$ 0.030 $&$ 0.078 $&$ 0.889$\\
$   35. $&$    0.727 \times 10^{-3} $&$ 0.041 $&$ 0.144 $&$ 0.232 $&$ 0.065 $&$ 0.281 $&$ 1.419 $&$ 0.038 $&$ 0.048 $&$ 0.020 $&$ 0.065 $&$ 0.884$\\
$   35. $&$    0.812 \times 10^{-3} $&$ 0.106 $&$ 0.075 $&$ 0.107 $&$ 0.054 $&$ 0.142 $&$ 1.411 $&$ 0.026 $&$ 0.027 $&$ 0.019 $&$ 0.042 $&$ 0.753$\\
$   35. $&$    0.921 \times 10^{-3} $&$ 0.436 $&$ 0.080 $&$ 0.125 $&$ 0.040 $&$ 0.153 $&$ 1.405 $&$ 0.022 $&$ 0.024 $&$ 0.014 $&$ 0.035 $&$ 0.727$\\
$   35. $&$    0.106 \times 10^{-2} $&$ 0.196 $&$ 0.072 $&$ 0.130 $&$ 0.042 $&$ 0.155 $&$ 1.325 $&$ 0.017 $&$ 0.021 $&$ 0.012 $&$ 0.030 $&$ 0.698$\\
$   35. $&$    0.141 \times 10^{-2} $&$ 0.057 $&$ 0.067 $&$ 0.170 $&$ 0.065 $&$ 0.194 $&$ 1.226 $&$ 0.008 $&$ 0.015 $&$ 0.011 $&$ 0.021 $&$ 0.639$\\
$   45. $&$    0.837 \times 10^{-3} $&$ 0.179 $&$ 0.117 $&$ 0.188 $&$ 0.061 $&$ 0.230 $&$ 1.518 $&$ 0.042 $&$ 0.054 $&$ 0.022 $&$ 0.072 $&$ 0.875$\\
$   45. $&$    0.934 \times 10^{-3} $&$ 0.516 $&$ 0.167 $&$ 0.238 $&$ 0.058 $&$ 0.296 $&$ 1.517 $&$ 0.043 $&$ 0.052 $&$ 0.022 $&$ 0.071 $&$ 0.869$\\
$   45. $&$    0.104 \times 10^{-2} $&$ 0.366 $&$ 0.084 $&$ 0.107 $&$ 0.054 $&$ 0.146 $&$ 1.430 $&$ 0.029 $&$ 0.027 $&$ 0.016 $&$ 0.042 $&$ 0.731$\\
$   45. $&$    0.118 \times 10^{-2} $&$ 0.396 $&$ 0.108 $&$ 0.118 $&$ 0.042 $&$ 0.165 $&$ 1.395 $&$ 0.025 $&$ 0.025 $&$ 0.014 $&$ 0.038 $&$ 0.732$\\
$   45. $&$    0.137 \times 10^{-2} $&$ 0.255 $&$ 0.100 $&$ 0.151 $&$ 0.047 $&$ 0.187 $&$ 1.350 $&$ 0.021 $&$ 0.023 $&$ 0.013 $&$ 0.034 $&$ 0.729$\\
$   45. $&$    0.181 \times 10^{-2} $&$ 0.099 $&$ 0.075 $&$ 0.175 $&$ 0.065 $&$ 0.202 $&$ 1.210 $&$ 0.009 $&$ 0.016 $&$ 0.011 $&$ 0.021 $&$ 0.659$\\
$   60. $&$    0.112 \times 10^{-2} $&$ 0.282 $&$ 0.146 $&$ 0.179 $&$ 0.051 $&$ 0.237 $&$ 1.446 $&$ 0.058 $&$ 0.058 $&$ 0.021 $&$ 0.084 $&$ 0.851$\\
$   60. $&$    0.125 \times 10^{-2} $&$ 0.279 $&$ 0.165 $&$ 0.198 $&$ 0.055 $&$ 0.263 $&$ 1.548 $&$ 0.048 $&$ 0.050 $&$ 0.018 $&$ 0.072 $&$ 0.844$\\
$   60. $&$    0.139 \times 10^{-2} $&$ 0.383 $&$ 0.095 $&$ 0.105 $&$ 0.049 $&$ 0.150 $&$ 1.450 $&$ 0.033 $&$ 0.030 $&$ 0.016 $&$ 0.047 $&$ 0.731$\\
$   60. $&$    0.158 \times 10^{-2} $&$ 0.464 $&$ 0.102 $&$ 0.101 $&$ 0.047 $&$ 0.151 $&$ 1.369 $&$ 0.027 $&$ 0.024 $&$ 0.014 $&$ 0.039 $&$ 0.711$\\
$   60. $&$    0.182 \times 10^{-2} $&$ 0.159 $&$ 0.230 $&$ 0.320 $&$ 0.047 $&$ 0.397 $&$ 1.288 $&$ 0.028 $&$ 0.033 $&$ 0.012 $&$ 0.045 $&$ 0.818$\\
$   60. $&$    0.242 \times 10^{-2} $&$-0.044 $&$ 0.094 $&$ 0.185 $&$ 0.069 $&$ 0.218 $&$ 1.186 $&$ 0.011 $&$ 0.016 $&$ 0.011 $&$ 0.023 $&$ 0.683$\\
$   90. $&$    0.187 \times 10^{-2} $&$ 0.041 $&$ 0.222 $&$ 0.207 $&$ 0.045 $&$ 0.307 $&$ 1.330 $&$ 0.095 $&$ 0.077 $&$ 0.017 $&$ 0.123 $&$ 0.862$\\
$   90. $&$    0.209 \times 10^{-2} $&$ 0.060 $&$ 0.109 $&$ 0.119 $&$ 0.041 $&$ 0.166 $&$ 1.313 $&$ 0.051 $&$ 0.045 $&$ 0.014 $&$ 0.069 $&$ 0.801$\\
$   90. $&$    0.237 \times 10^{-2} $&$ 0.007 $&$ 0.109 $&$ 0.101 $&$ 0.040 $&$ 0.154 $&$ 1.218 $&$ 0.037 $&$ 0.029 $&$ 0.012 $&$ 0.048 $&$ 0.769$\\
$   90. $&$    0.273 \times 10^{-2} $&$ 0.447 $&$ 0.143 $&$ 0.135 $&$ 0.048 $&$ 0.202 $&$ 1.325 $&$ 0.031 $&$ 0.027 $&$ 0.013 $&$ 0.043 $&$ 0.717$\\
$   90. $&$    0.362 \times 10^{-2} $&$ 0.163 $&$ 0.167 $&$ 0.233 $&$ 0.058 $&$ 0.293 $&$ 1.145 $&$ 0.015 $&$ 0.017 $&$ 0.011 $&$ 0.025 $&$ 0.699$\\
$  120. $&$    0.220 \times 10^{-2} $&$ 0.070 $&$ 0.067 $&$ 0.241 $&$ 0.041 $&$ 0.253 $&$ 1.400 $&$ 0.019 $&$ 0.060 $&$ 0.027 $&$ 0.069 $&$ 0.908$\\
$  120. $&$    0.250 \times 10^{-2} $&$ 0.450 $&$ 0.096 $&$ 0.252 $&$ 0.037 $&$ 0.272 $&$ 1.414 $&$ 0.022 $&$ 0.051 $&$ 0.025 $&$ 0.061 $&$ 0.875$\\
$  120. $&$    0.280 \times 10^{-2} $&$ 0.136 $&$ 0.094 $&$ 0.103 $&$ 0.036 $&$ 0.144 $&$ 1.299 $&$ 0.022 $&$ 0.025 $&$ 0.021 $&$ 0.039 $&$ 0.711$\\
$  120. $&$    0.320 \times 10^{-2} $&$ 0.073 $&$ 0.175 $&$ 0.342 $&$ 0.032 $&$ 0.385 $&$ 1.129 $&$ 0.103 $&$ 0.146 $&$ 0.018 $&$ 0.179 $&$ 0.963$\\
$  120. $&$    0.360 \times 10^{-2} $&$ 0.480 $&$ 0.178 $&$ 0.234 $&$ 0.039 $&$ 0.296 $&$ 1.245 $&$ 0.062 $&$ 0.063 $&$ 0.012 $&$ 0.089 $&$ 0.886$\\
$  120. $&$    0.480 \times 10^{-2} $&$ 0.152 $&$ 0.166 $&$ 0.212 $&$ 0.071 $&$ 0.278 $&$ 1.069 $&$ 0.024 $&$ 0.024 $&$ 0.010 $&$ 0.035 $&$ 0.762$\\
$  150. $&$    0.280 \times 10^{-2} $&$ 0.123 $&$ 0.083 $&$ 0.270 $&$ 0.046 $&$ 0.286 $&$ 1.357 $&$ 0.024 $&$ 0.065 $&$ 0.025 $&$ 0.074 $&$ 0.931$\\
$  150. $&$    0.310 \times 10^{-2} $&$ 0.306 $&$ 0.099 $&$ 0.290 $&$ 0.035 $&$ 0.308 $&$ 1.330 $&$ 0.022 $&$ 0.056 $&$ 0.023 $&$ 0.065 $&$ 0.904$\\
$  150. $&$    0.350 \times 10^{-2} $&$ 0.038 $&$ 0.085 $&$ 0.127 $&$ 0.038 $&$ 0.157 $&$ 1.274 $&$ 0.017 $&$ 0.027 $&$ 0.021 $&$ 0.038 $&$ 0.728$\\
$  150. $&$    0.390 \times 10^{-2} $&$ 0.401 $&$ 0.095 $&$ 0.124 $&$ 0.029 $&$ 0.159 $&$ 1.266 $&$ 0.015 $&$ 0.022 $&$ 0.020 $&$ 0.033 $&$ 0.675$\\
$  150. $&$    0.450 \times 10^{-2} $&$ 0.554 $&$ 0.114 $&$ 0.153 $&$ 0.038 $&$ 0.195 $&$ 1.209 $&$ 0.014 $&$ 0.023 $&$ 0.020 $&$ 0.034 $&$ 0.668$\\
$  150. $&$    0.600 \times 10^{-2} $&$ 0.137 $&$ 0.118 $&$ 0.194 $&$ 0.060 $&$ 0.235 $&$ 1.069 $&$ 0.009 $&$ 0.020 $&$ 0.018 $&$ 0.028 $&$ 0.677$\\
$  200. $&$    0.370 \times 10^{-2} $&$-0.039 $&$ 0.110 $&$ 0.305 $&$ 0.044 $&$ 0.327 $&$ 1.231 $&$ 0.033 $&$ 0.072 $&$ 0.023 $&$ 0.083 $&$ 0.944$\\
$  200. $&$    0.410 \times 10^{-2} $&$-0.157 $&$ 0.141 $&$ 0.321 $&$ 0.033 $&$ 0.352 $&$ 1.160 $&$ 0.032 $&$ 0.059 $&$ 0.020 $&$ 0.070 $&$ 0.929$\\
$  200. $&$    0.460 \times 10^{-2} $&$ 0.146 $&$ 0.115 $&$ 0.131 $&$ 0.038 $&$ 0.179 $&$ 1.188 $&$ 0.023 $&$ 0.025 $&$ 0.019 $&$ 0.039 $&$ 0.758$\\
$  200. $&$    0.520 \times 10^{-2} $&$ 0.184 $&$ 0.126 $&$ 0.138 $&$ 0.033 $&$ 0.189 $&$ 1.136 $&$ 0.019 $&$ 0.022 $&$ 0.019 $&$ 0.035 $&$ 0.719$\\
$  200. $&$    0.610 \times 10^{-2} $&$ 0.253 $&$ 0.141 $&$ 0.169 $&$ 0.033 $&$ 0.223 $&$ 1.107 $&$ 0.016 $&$ 0.021 $&$ 0.018 $&$ 0.032 $&$ 0.690$\\
$  200. $&$    0.800 \times 10^{-2} $&$ 0.228 $&$ 0.126 $&$ 0.203 $&$ 0.057 $&$ 0.246 $&$ 0.995 $&$ 0.008 $&$ 0.018 $&$ 0.017 $&$ 0.026 $&$ 0.654$\\
$  250. $&$    0.460 \times 10^{-2} $&$ 0.620 $&$ 0.136 $&$ 0.365 $&$ 0.052 $&$ 0.393 $&$ 1.340 $&$ 0.041 $&$ 0.086 $&$ 0.025 $&$ 0.099 $&$ 0.950$\\
$  250. $&$    0.520 \times 10^{-2} $&$ 0.214 $&$ 0.159 $&$ 0.349 $&$ 0.039 $&$ 0.385 $&$ 1.186 $&$ 0.037 $&$ 0.065 $&$ 0.020 $&$ 0.077 $&$ 0.931$\\
$  250. $&$    0.580 \times 10^{-2} $&$ 0.243 $&$ 0.130 $&$ 0.142 $&$ 0.038 $&$ 0.196 $&$ 1.176 $&$ 0.026 $&$ 0.027 $&$ 0.019 $&$ 0.041 $&$ 0.770$\\
$  250. $&$    0.660 \times 10^{-2} $&$ 0.163 $&$ 0.145 $&$ 0.146 $&$ 0.030 $&$ 0.208 $&$ 1.087 $&$ 0.022 $&$ 0.022 $&$ 0.016 $&$ 0.035 $&$ 0.742$\\
$  250. $&$    0.760 \times 10^{-2} $&$ 0.117 $&$ 0.159 $&$ 0.173 $&$ 0.031 $&$ 0.237 $&$ 0.998 $&$ 0.018 $&$ 0.020 $&$ 0.016 $&$ 0.032 $&$ 0.714$\\
$  250. $&$    0.100 \times 10^{-1} $&$ 0.105 $&$ 0.139 $&$ 0.197 $&$ 0.050 $&$ 0.246 $&$ 0.914 $&$ 0.008 $&$ 0.015 $&$ 0.015 $&$ 0.023 $&$ 0.650$\\
$  250. $&$    0.130 \times 10^{-1} $&$ 0.140 $&$ 0.228 $&$ 0.280 $&$ 0.095 $&$ 0.374 $&$ 0.842 $&$ 0.008 $&$ 0.014 $&$ 0.014 $&$ 0.021 $&$ 0.650$\\
$  300. $&$    0.560 \times 10^{-2} $&$-0.038 $&$ 0.161 $&$ 0.316 $&$ 0.041 $&$ 0.357 $&$ 1.138 $&$ 0.048 $&$ 0.075 $&$ 0.021 $&$ 0.091 $&$ 0.942$\\
$  300. $&$    0.690 \times 10^{-2} $&$ 0.345 $&$ 0.151 $&$ 0.149 $&$ 0.039 $&$ 0.216 $&$ 1.118 $&$ 0.030 $&$ 0.028 $&$ 0.019 $&$ 0.045 $&$ 0.781$\\
$  300. $&$    0.790 \times 10^{-2} $&$ 0.377 $&$ 0.168 $&$ 0.148 $&$ 0.027 $&$ 0.225 $&$ 1.058 $&$ 0.025 $&$ 0.022 $&$ 0.016 $&$ 0.037 $&$ 0.752$\\
$  300. $&$    0.910 \times 10^{-2} $&$ 0.349 $&$ 0.193 $&$ 0.176 $&$ 0.028 $&$ 0.263 $&$ 0.967 $&$ 0.021 $&$ 0.019 $&$ 0.015 $&$ 0.033 $&$ 0.734$\\
$  300. $&$    0.121 \times 10^{-1} $&$-0.324 $&$ 0.157 $&$ 0.200 $&$ 0.047 $&$ 0.258 $&$ 0.839 $&$ 0.009 $&$ 0.014 $&$ 0.014 $&$ 0.022 $&$ 0.663$\\
$  400. $&$    0.930 \times 10^{-2} $&$-0.093 $&$ 0.164 $&$ 0.135 $&$ 0.033 $&$ 0.215 $&$ 0.950 $&$ 0.033 $&$ 0.025 $&$ 0.015 $&$ 0.044 $&$ 0.790$\\
$  400. $&$    0.105 \times 10^{-1} $&$-0.199 $&$ 0.180 $&$ 0.131 $&$ 0.020 $&$ 0.223 $&$ 0.923 $&$ 0.028 $&$ 0.019 $&$ 0.014 $&$ 0.037 $&$ 0.760$\\
$  400. $&$    0.121 \times 10^{-1} $&$-0.051 $&$ 0.207 $&$ 0.179 $&$ 0.027 $&$ 0.275 $&$ 0.913 $&$ 0.023 $&$ 0.021 $&$ 0.015 $&$ 0.034 $&$ 0.736$\\
$  400. $&$    0.161 \times 10^{-1} $&$-0.180 $&$ 0.182 $&$ 0.202 $&$ 0.043 $&$ 0.276 $&$ 0.788 $&$ 0.011 $&$ 0.013 $&$ 0.012 $&$ 0.021 $&$ 0.680$\\
$  500. $&$    0.116 \times 10^{-1} $&$-0.255 $&$ 0.184 $&$ 0.119 $&$ 0.028 $&$ 0.221 $&$ 0.868 $&$ 0.037 $&$ 0.022 $&$ 0.014 $&$ 0.046 $&$ 0.790$\\
$  500. $&$    0.131 \times 10^{-1} $&$ 0.340 $&$ 0.207 $&$ 0.143 $&$ 0.019 $&$ 0.252 $&$ 0.946 $&$ 0.033 $&$ 0.022 $&$ 0.015 $&$ 0.042 $&$ 0.755$\\
$  500. $&$    0.152 \times 10^{-1} $&$ 0.279 $&$ 0.244 $&$ 0.149 $&$ 0.021 $&$ 0.287 $&$ 0.860 $&$ 0.028 $&$ 0.017 $&$ 0.012 $&$ 0.035 $&$ 0.742$\\
$  500. $&$    0.201 \times 10^{-1} $&$ 0.192 $&$ 0.214 $&$ 0.211 $&$ 0.043 $&$ 0.304 $&$ 0.770 $&$ 0.013 $&$ 0.014 $&$ 0.013 $&$ 0.023 $&$ 0.691$\\
$  650. $&$    0.151 \times 10^{-1} $&$ 0.229 $&$ 0.219 $&$ 0.145 $&$ 0.018 $&$ 0.263 $&$ 0.917 $&$ 0.043 $&$ 0.026 $&$ 0.013 $&$ 0.052 $&$ 0.804$\\
$  650. $&$    0.171 \times 10^{-1} $&$-0.229 $&$ 0.209 $&$ 0.132 $&$ 0.016 $&$ 0.248 $&$ 0.743 $&$ 0.033 $&$ 0.021 $&$ 0.012 $&$ 0.041 $&$ 0.769$\\
$  650. $&$    0.197 \times 10^{-1} $&$-0.204 $&$ 0.254 $&$ 0.148 $&$ 0.019 $&$ 0.294 $&$ 0.735 $&$ 0.030 $&$ 0.017 $&$ 0.011 $&$ 0.036 $&$ 0.750$\\
$  650. $&$    0.261 \times 10^{-1} $&$ 0.651 $&$ 0.244 $&$ 0.201 $&$ 0.036 $&$ 0.318 $&$ 0.739 $&$ 0.016 $&$ 0.014 $&$ 0.012 $&$ 0.024 $&$ 0.698$\\
$  800. $&$    0.185 \times 10^{-1} $&$ 0.625 $&$ 0.228 $&$ 0.158 $&$ 0.014 $&$ 0.278 $&$ 0.821 $&$ 0.045 $&$ 0.028 $&$ 0.013 $&$ 0.054 $&$ 0.812$\\
$  800. $&$    0.210 \times 10^{-1} $&$ 0.205 $&$ 0.230 $&$ 0.167 $&$ 0.015 $&$ 0.285 $&$ 0.762 $&$ 0.036 $&$ 0.026 $&$ 0.012 $&$ 0.046 $&$ 0.774$\\
$  800. $&$    0.242 \times 10^{-1} $&$ 0.123 $&$ 0.281 $&$ 0.148 $&$ 0.016 $&$ 0.318 $&$ 0.698 $&$ 0.033 $&$ 0.017 $&$ 0.010 $&$ 0.039 $&$ 0.753$\\
$  800. $&$    0.322 \times 10^{-1} $&$ 0.276 $&$ 0.253 $&$ 0.202 $&$ 0.031 $&$ 0.325 $&$ 0.642 $&$ 0.016 $&$ 0.014 $&$ 0.010 $&$ 0.023 $&$ 0.714$\\
\hline 
\end{tabular} 
\end{center} 
%% \caption{\label{tab:flf2a} The proton structure functions $F_L$ and $F_2$
%% measured at the given values of $Q^2$ and $x$ without model assumptions.
%% $\Delta_{\rm stat}F_{L}$, $\Delta_{\rm uncor}F_{L}$,
%% $\Delta_{\rm cor}F_{L}$ and $\Delta_{\rm tot}F_{L}$
%% are the statistical, uncorrelated systematic, correlated systematic, and total uncertainty on $F_L$
%% respectively.
%% $\Delta_{\rm stat}F_{2}$, $\Delta_{\rm uncor}F_{2}$,
%% $\Delta_{\rm cor}F_{2}$ and $\Delta_{\rm tot}F_{2}$
%% are the statistical, uncorrelated systematic and total uncertainty on $F_2$,
%% respectively.
%% $\rho$ is the correlation coefficient between the $F_L$ and $F_2$ values.}
\caption{\label{tab:flf2b} Continued from table~\ref{tab:flf2a}. } 
\end{table} 



==> plots/xsec460.tex <==
\begin{table}[htbp] 
\begin{center} 
\tiny 
\begin{tabular}{|r|c|c|r|r|r|r|r|r|r|r|r|r|r|r|r|} 
\hline 
$Q^2$ & $x$ & $y$ & $\tilde{\sigma}_{\rm NC}$ & 
$\delta_{\rm tot}$ & $\delta_{\rm stat}$ & $\delta_{\rm unc}$ & 
$\delta_{\rm unc}^{E}$ & 
$\delta_{\rm unc}^{h}$& 
$\delta_{\rm cor}$ & 
$\delta_{\rm cor}^{E^+}$ & 
$\delta_{\rm cor}^{\theta^+}$& 
$\delta_{\rm cor}^{h^+}$& 
$\delta_{\rm cor}^{N^+}$& 
$\delta_{\rm cor}^{S^+}$& 
$\delta_{\rm cor}^{D^+}$ \\ 
$(\rm GeV^2)$ & & & & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ 
\\ \hline 
$35$ & $8.10 \times 10^{-4}$ & $0.850$ & $1.343$ & $6.5$ & $4.5$ & $3.8$ & $0.6$ & $2.8$ & $2.8$ & $-0.3$ & $-0.4$ & $0.2$ & $0.7$ & $2.3$ & $1.2$ \\ 
 
\hline 
$45$ & $1.04 \times 10^{-3}$ & $0.850$ & $1.173$ & $6.3$ & $4.7$ & $3.4$ & $0.4$ & $2.4$ & $2.4$ & $-0.1$ & $-0.5$ & $0.1$ & $0.6$ & $2.1$ & $1.0$ \\ 
 
$45$ & $1.18 \times 10^{-3}$ & $0.750$ & $1.187$ & $5.7$ & $5.1$ & $2.2$ & $0.6$ & $0.8$ & $1.3$ & $0.2$ & $-0.5$ & $0.0$ & $0.3$ & $0.6$ & $1.0$ \\ 
 
\hline 
$60$ & $1.39 \times 10^{-3}$ & $0.850$ & $1.190$ & $6.2$ & $5.0$ & $3.0$ & $0.2$ & $2.0$ & $2.0$ & $-0.1$ & $-0.3$ & $0.1$ & $0.5$ & $1.7$ & $0.8$ \\ 
 
$60$ & $1.58 \times 10^{-3}$ & $0.750$ & $1.117$ & $4.7$ & $4.0$ & $2.0$ & $0.5$ & $0.6$ & $1.4$ & $-0.2$ & $-0.6$ & $0.0$ & $0.2$ & $0.6$ & $1.0$ \\ 
 
\hline 
$90$ & $2.09 \times 10^{-3}$ & $0.850$ & $1.269$ & $6.3$ & $5.3$ & $2.9$ & $0.3$ & $1.8$ & $1.8$ & $-0.2$ & $-0.4$ & $0.1$ & $0.5$ & $1.4$ & $0.9$ \\ 
 
$90$ & $2.36 \times 10^{-3}$ & $0.750$ & $1.193$ & $4.6$ & $4.1$ & $1.9$ & $0.3$ & $0.5$ & $1.1$ & $-0.2$ & $-0.5$ & $0.1$ & $0.2$ & $0.3$ & $0.9$ \\ 
 
$90$ & $2.73 \times 10^{-3}$ & $0.650$ & $1.156$ & $4.2$ & $3.8$ & $1.8$ & $0.4$ & $0.2$ & $0.8$ & $-0.2$ & $-0.6$ & $0.0$ & $0.2$ & $0.3$ & $0.4$ \\ 
 
\hline 
$120$ & $2.78 \times 10^{-3}$ & $0.850$ & $1.249$ & $6.8$ & $6.1$ & $2.7$ & $0.1$ & $1.5$ & $1.6$ & $0.0$ & $-0.4$ & $0.1$ & $0.4$ & $0.9$ & $1.2$ \\ 
 
$120$ & $3.15 \times 10^{-3}$ & $0.750$ & $1.099$ & $5.3$ & $4.8$ & $1.9$ & $0.4$ & $0.4$ & $0.9$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.4$ & $0.6$ \\ 
 
$120$ & $3.63 \times 10^{-3}$ & $0.650$ & $1.052$ & $4.7$ & $4.3$ & $1.9$ & $0.6$ & $0.2$ & $0.6$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.2$ & $0.2$ \\ 
 
$120$ & $4.82 \times 10^{-3}$ & $0.490$ & $1.041$ & $3.3$ & $2.7$ & $1.8$ & $0.6$ & $0.1$ & $0.8$ & $-0.3$ & $-0.7$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
\hline 
$150$ & $3.47 \times 10^{-3}$ & $0.850$ & $1.230$ & $7.8$ & $7.1$ & $2.6$ & $0.4$ & $1.4$ & $1.9$ & $-0.2$ & $-0.3$ & $0.1$ & $0.4$ & $0.8$ & $1.6$ \\ 
 
$150$ & $3.94 \times 10^{-3}$ & $0.750$ & $1.024$ & $6.1$ & $5.8$ & $1.9$ & $0.4$ & $0.3$ & $0.8$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.2$ & $0.6$ \\ 
 
$150$ & $4.54 \times 10^{-3}$ & $0.650$ & $1.010$ & $5.4$ & $5.0$ & $2.0$ & $0.9$ & $0.1$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.2$ & $0.1$ \\ 
 
$150$ & $6.03 \times 10^{-3}$ & $0.490$ & $1.060$ & $3.2$ & $2.5$ & $1.8$ & $0.5$ & $0.1$ & $0.7$ & $-0.3$ & $-0.6$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$150$ & $8.00 \times 10^{-3}$ & $0.369$ & $0.9774$ & $3.0$ & $2.6$ & $1.4$ & $0.6$ & $0.0$ & $0.9$ & $-0.4$ & $-0.8$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$150$ & $1.30 \times 10^{-2}$ & $0.227$ & $0.8384$ & $3.8$ & $3.3$ & $1.5$ & $1.2$ & $0.0$ & $1.1$ & $-0.8$ & $-0.7$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$150$ & $2.00 \times 10^{-2}$ & $0.148$ & $0.7006$ & $5.2$ & $4.5$ & $2.2$ & $1.7$ & $1.0$ & $1.7$ & $-1.0$ & $-1.0$ & $-0.4$ & $-0.8$ & $0.0$ & $0.0$ \\ 
 
\hline 
$200$ & $4.63 \times 10^{-3}$ & $0.850$ & $1.117$ & $9.6$ & $9.1$ & $2.5$ & $0.3$ & $1.1$ & $2.1$ & $-0.1$ & $-0.4$ & $0.0$ & $0.3$ & $0.6$ & $1.9$ \\ 
 
$200$ & $5.25 \times 10^{-3}$ & $0.750$ & $1.011$ & $8.1$ & $7.7$ & $1.9$ & $0.3$ & $0.3$ & $1.1$ & $0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.1$ & $1.0$ \\ 
 
$200$ & $6.06 \times 10^{-3}$ & $0.650$ & $0.9997$ & $6.8$ & $6.5$ & $2.0$ & $0.9$ & $0.2$ & $0.6$ & $-0.1$ & $-0.5$ & $0.1$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$200$ & $8.04 \times 10^{-3}$ & $0.490$ & $0.9567$ & $3.8$ & $3.4$ & $1.7$ & $0.3$ & $0.1$ & $0.6$ & $-0.3$ & $-0.6$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$200$ & $1.30 \times 10^{-2}$ & $0.303$ & $0.8430$ & $3.4$ & $3.1$ & $1.0$ & $0.6$ & $0.0$ & $0.8$ & $-0.4$ & $-0.7$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$200$ & $2.00 \times 10^{-2}$ & $0.197$ & $0.6517$ & $4.1$ & $3.5$ & $1.8$ & $1.6$ & $0.0$ & $1.2$ & $-1.0$ & $-0.7$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$200$ & $3.20 \times 10^{-2}$ & $0.123$ & $0.5275$ & $4.2$ & $4.0$ & $0.9$ & $0.1$ & $0.1$ & $0.6$ & $-0.1$ & $-0.5$ & $-0.1$ & $0.3$ & $0.0$ & $0.0$ \\ 
 
$200$ & $5.00 \times 10^{-2}$ & $0.079$ & $0.5297$ & $4.3$ & $4.1$ & $1.2$ & $0.9$ & $0.2$ & $0.7$ & $-0.5$ & $-0.4$ & $-0.1$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$200$ & $8.00 \times 10^{-2}$ & $0.049$ & $0.4587$ & $5.0$ & $4.7$ & $1.3$ & $0.9$ & $0.3$ & $1.0$ & $-0.6$ & $-0.7$ & $-0.2$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$200$ & $1.30 \times 10^{-1}$ & $0.030$ & $0.3610$ & $5.6$ & $5.1$ & $1.9$ & $1.5$ & $0.1$ & $1.6$ & $-0.9$ & $-0.7$ & $-0.1$ & $1.0$ & $0.0$ & $0.0$ \\ 
 
$200$ & $1.80 \times 10^{-1}$ & $0.022$ & $0.3201$ & $6.8$ & $5.8$ & $2.3$ & $1.1$ & $1.4$ & $2.6$ & $-0.7$ & $-0.9$ & $-0.4$ & $-2.3$ & $0.0$ & $0.0$ \\ 
 
$200$ & $4.00 \times 10^{-1}$ & $0.010$ & $0.1694$ & $13.1$ & $8.2$ & $4.5$ & $0.3$ & $4.0$ & $9.2$ & $0.2$ & $-1.1$ & $-0.6$ & $-9.1$ & $0.0$ & $0.0$ \\ 
 
\hline 
$250$ & $5.79 \times 10^{-3}$ & $0.850$ & $1.049$ & $10.9$ & $10.4$ & $2.5$ & $0.3$ & $0.9$ & $2.2$ & $-0.1$ & $-0.2$ & $0.0$ & $0.3$ & $0.6$ & $2.0$ \\ 
 
$250$ & $6.56 \times 10^{-3}$ & $0.750$ & $1.036$ & $9.1$ & $8.8$ & $1.9$ & $0.2$ & $0.3$ & $1.3$ & $-0.2$ & $-0.4$ & $0.1$ & $0.2$ & $0.2$ & $1.1$ \\ 
 
$250$ & $7.57 \times 10^{-3}$ & $0.650$ & $0.9480$ & $8.0$ & $7.7$ & $2.0$ & $0.9$ & $0.1$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$250$ & $1.00 \times 10^{-2}$ & $0.490$ & $0.8829$ & $4.3$ & $3.9$ & $1.7$ & $0.3$ & $0.1$ & $0.6$ & $-0.3$ & $-0.5$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$250$ & $1.30 \times 10^{-2}$ & $0.379$ & $0.8281$ & $4.0$ & $3.7$ & $1.3$ & $0.4$ & $0.0$ & $0.6$ & $-0.4$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$250$ & $2.00 \times 10^{-2}$ & $0.246$ & $0.6799$ & $4.0$ & $3.8$ & $1.0$ & $0.6$ & $0.0$ & $0.8$ & $-0.5$ & $-0.7$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$250$ & $3.20 \times 10^{-2}$ & $0.154$ & $0.5817$ & $4.4$ & $4.1$ & $1.3$ & $1.0$ & $0.2$ & $0.9$ & $0.4$ & $-0.6$ & $0.1$ & $0.6$ & $0.0$ & $0.0$ \\ 
 
$250$ & $5.00 \times 10^{-2}$ & $0.098$ & $0.5025$ & $4.4$ & $4.1$ & $1.3$ & $0.9$ & $0.1$ & $0.9$ & $0.3$ & $-0.6$ & $0.0$ & $0.7$ & $0.0$ & $0.0$ \\ 
 
$250$ & $8.00 \times 10^{-2}$ & $0.062$ & $0.4429$ & $4.7$ & $4.4$ & $1.3$ & $1.0$ & $0.1$ & $1.0$ & $0.5$ & $-0.6$ & $-0.1$ & $0.7$ & $0.0$ & $0.0$ \\ 
 
$250$ & $1.30 \times 10^{-1}$ & $0.038$ & $0.3750$ & $4.9$ & $4.4$ & $1.4$ & $0.8$ & $0.1$ & $1.6$ & $0.3$ & $-0.5$ & $-0.1$ & $1.5$ & $0.0$ & $0.0$ \\ 
 
$250$ & $1.80 \times 10^{-1}$ & $0.027$ & $0.3582$ & $5.1$ & $4.5$ & $2.1$ & $1.3$ & $0.9$ & $1.3$ & $0.6$ & $-0.7$ & $-0.3$ & $-0.8$ & $0.0$ & $0.0$ \\ 
 
$250$ & $4.00 \times 10^{-1}$ & $0.012$ & $0.1675$ & $12.6$ & $6.6$ & $4.9$ & $2.7$ & $3.6$ & $9.5$ & $1.6$ & $-1.0$ & $-0.6$ & $-9.3$ & $0.0$ & $0.0$ \\ 
 
\hline 
$300$ & $6.95 \times 10^{-3}$ & $0.850$ & $0.8700$ & $13.8$ & $13.3$ & $2.4$ & $0.2$ & $0.8$ & $2.5$ & $-0.2$ & $-0.2$ & $0.0$ & $0.3$ & $0.8$ & $2.3$ \\ 
 
$300$ & $7.88 \times 10^{-3}$ & $0.750$ & $0.8274$ & $11.1$ & $10.9$ & $2.0$ & $0.2$ & $0.3$ & $1.0$ & $-0.2$ & $-0.3$ & $0.0$ & $0.2$ & $0.3$ & $0.9$ \\ 
 
$300$ & $9.09 \times 10^{-3}$ & $0.650$ & $0.8411$ & $9.8$ & $9.6$ & $1.9$ & $0.3$ & $0.1$ & $0.5$ & $0.1$ & $-0.4$ & $0.0$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$300$ & $1.21 \times 10^{-2}$ & $0.490$ & $0.9058$ & $4.8$ & $4.5$ & $1.7$ & $0.3$ & $0.1$ & $0.5$ & $-0.3$ & $-0.4$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$300$ & $2.00 \times 10^{-2}$ & $0.295$ & $0.7296$ & $4.4$ & $4.2$ & $1.0$ & $0.6$ & $0.0$ & $0.8$ & $-0.6$ & $-0.5$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$300$ & $3.20 \times 10^{-2}$ & $0.185$ & $0.6231$ & $4.7$ & $4.5$ & $0.9$ & $0.3$ & $0.2$ & $0.7$ & $0.3$ & $-0.3$ & $0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$300$ & $5.00 \times 10^{-2}$ & $0.118$ & $0.5210$ & $4.9$ & $4.7$ & $1.1$ & $0.6$ & $0.2$ & $0.9$ & $0.4$ & $-0.5$ & $0.1$ & $0.6$ & $0.0$ & $0.0$ \\ 
 
$300$ & $8.00 \times 10^{-2}$ & $0.074$ & $0.4584$ & $5.2$ & $4.9$ & $1.4$ & $1.0$ & $0.2$ & $1.0$ & $0.6$ & $-0.6$ & $-0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$300$ & $1.30 \times 10^{-1}$ & $0.045$ & $0.3695$ & $5.5$ & $5.1$ & $1.5$ & $1.0$ & $0.2$ & $1.6$ & $0.5$ & $-0.6$ & $0.0$ & $1.4$ & $0.0$ & $0.0$ \\ 
 
$300$ & $1.80 \times 10^{-1}$ & $0.033$ & $0.3330$ & $5.8$ & $5.2$ & $2.2$ & $1.5$ & $0.9$ & $1.2$ & $0.9$ & $-0.8$ & $-0.3$ & $-0.3$ & $0.0$ & $0.0$ \\ 
 
$300$ & $4.00 \times 10^{-1}$ & $0.015$ & $0.1567$ & $13.0$ & $7.7$ & $5.2$ & $3.1$ & $3.6$ & $9.1$ & $2.1$ & $-1.3$ & $-0.6$ & $-8.8$ & $0.0$ & $0.0$ \\ 
 
\hline 

\end{tabular} 
\end{center} 
\caption[RESULT] 
{\sl \label{tab:xsec460} The NC 
$e^+p$ reduced cross section $\tilde{\sigma}_{\rm NC}(x,Q^2)$ 
for $E_p=460$ GeV and $P_e=0$ 
with statistical 
$(\delta_{\rm stat})$, 
total $(\delta_{tot})$, 
total uncorrelated systematic $(\delta_{\rm unc})$ 
errors, two of its contributions from the 
 electron energy error ($\delta_{unc}^{E}$)  
and the hadronic energy error  
($\delta_{\rm unc}^{h}$). 
The effect of the other uncorrelated 
systematic errors is included in $\delta_{\rm unc}$. 
In addition the correlated systematic  
$(\delta_{\rm cor})$ and its contributions from a 
positive variation of one  
standard deviation of the 
electron energy error ($\delta_{cor}^{E^+}$), of 
the polar electron angle error 
($\delta_{\rm cor}^{\theta^+}$), of the hadronic 
energy error ($\delta_{\rm cor}^{h^+}$), of the error 
due to noise subtraction ($\delta_{\rm cor}^{N^+}$), 
of the error 
due to background subtraction charge asymmetry 
 ($\delta_{\rm cor}^{S^+}$) 
and of the error 
due to variation of the cut value on the electron discriminator $D_{ele}$  
 ($\delta_{\rm cor}^{D^+}$) are given. 
The normalisation uncertainty is 
not included in the errors. 
The table continues on the next page.}
\end{table} 
\begin{table}[htbp] 
\begin{center} 
\tiny 
\begin{tabular}{|r|c|c|r|r|r|r|r|r|r|r|r|r|r|r|r|} 
\hline 
$Q^2$ & $x$ & $y$ & $\tilde{\sigma}_{\rm NC}$ & 
$\delta_{\rm tot}$ & $\delta_{\rm stat}$ & $\delta_{\rm unc}$ & 
$\delta_{\rm unc}^{E}$ & 
$\delta_{\rm unc}^{h}$& 
$\delta_{\rm cor}$ & 
$\delta_{\rm cor}^{E^+}$ & 
$\delta_{\rm cor}^{\theta^+}$& 
$\delta_{\rm cor}^{h^+}$& 
$\delta_{\rm cor}^{N^+}$& 
$\delta_{\rm cor}^{S^+}$& 
$\delta_{\rm cor}^{D^+}$ \\ 
$(\rm GeV^2)$ & & & & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ 
\\ \hline 
$400$ & $9.27 \times 10^{-3}$ & $0.850$ & $1.025$ & $13.8$ & $13.3$ & $2.4$ & $0.6$ & $0.6$ & $2.5$ & $-0.2$ & $-0.3$ & $0.0$ & $0.2$ & $0.6$ & $2.4$ \\ 
 
$400$ & $1.05 \times 10^{-2}$ & $0.750$ & $1.074$ & $10.4$ & $10.1$ & $2.2$ & $1.0$ & $0.3$ & $0.7$ & $0.2$ & $-0.3$ & $0.1$ & $0.2$ & $0.1$ & $0.6$ \\ 
 
$400$ & $1.21 \times 10^{-2}$ & $0.650$ & $0.9263$ & $10.0$ & $9.8$ & $1.9$ & $0.2$ & $0.1$ & $0.4$ & $-0.2$ & $-0.3$ & $0.0$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$400$ & $1.61 \times 10^{-2}$ & $0.490$ & $0.8145$ & $5.7$ & $5.4$ & $1.7$ & $0.2$ & $0.0$ & $0.5$ & $-0.2$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$400$ & $3.20 \times 10^{-2}$ & $0.246$ & $0.6305$ & $5.2$ & $5.0$ & $1.0$ & $0.6$ & $0.0$ & $0.8$ & $-0.6$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$400$ & $5.00 \times 10^{-2}$ & $0.157$ & $0.5686$ & $5.4$ & $5.2$ & $1.0$ & $0.6$ & $0.2$ & $0.9$ & $0.5$ & $-0.5$ & $-0.1$ & $0.4$ & $0.0$ & $0.0$ \\ 
 
$400$ & $8.00 \times 10^{-2}$ & $0.098$ & $0.4493$ & $5.8$ & $5.7$ & $1.0$ & $0.4$ & $0.1$ & $0.7$ & $0.4$ & $-0.4$ & $0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$400$ & $1.30 \times 10^{-1}$ & $0.061$ & $0.4300$ & $5.6$ & $5.3$ & $1.2$ & $0.4$ & $0.1$ & $1.2$ & $0.4$ & $-0.4$ & $-0.1$ & $1.1$ & $0.0$ & $0.0$ \\ 
 
$400$ & $1.80 \times 10^{-1}$ & $0.044$ & $0.3375$ & $6.2$ & $5.8$ & $1.7$ & $0.8$ & $0.7$ & $0.9$ & $0.7$ & $-0.6$ & $-0.2$ & $-0.2$ & $0.0$ & $0.0$ \\ 
 
$400$ & $4.00 \times 10^{-1}$ & $0.020$ & $0.1494$ & $13.1$ & $8.7$ & $4.6$ & $1.9$ & $3.7$ & $8.6$ & $1.9$ & $-0.9$ & $-0.7$ & $-8.3$ & $0.0$ & $0.0$ \\ 
 
\hline 
$500$ & $1.16 \times 10^{-2}$ & $0.850$ & $1.002$ & $15.0$ & $14.6$ & $2.4$ & $0.1$ & $0.4$ & $2.2$ & $0.2$ & $-0.2$ & $0.0$ & $0.2$ & $0.0$ & $2.2$ \\ 
 
$500$ & $1.31 \times 10^{-2}$ & $0.750$ & $0.7577$ & $13.8$ & $13.6$ & $2.1$ & $0.6$ & $0.2$ & $0.5$ & $-0.3$ & $-0.3$ & $0.0$ & $0.2$ & $0.1$ & $0.1$ \\ 
 
$500$ & $1.51 \times 10^{-2}$ & $0.650$ & $0.6938$ & $12.4$ & $12.2$ & $1.9$ & $0.3$ & $0.1$ & $0.4$ & $-0.2$ & $-0.4$ & $0.1$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$500$ & $2.01 \times 10^{-2}$ & $0.490$ & $0.7395$ & $6.7$ & $6.5$ & $1.7$ & $0.1$ & $0.0$ & $0.4$ & $-0.1$ & $-0.4$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$500$ & $3.20 \times 10^{-2}$ & $0.308$ & $0.6559$ & $6.1$ & $6.0$ & $1.0$ & $0.3$ & $0.0$ & $0.6$ & $-0.3$ & $-0.5$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$500$ & $5.00 \times 10^{-2}$ & $0.197$ & $0.6106$ & $6.1$ & $5.9$ & $1.3$ & $0.9$ & $0.0$ & $1.1$ & $-0.9$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$500$ & $8.00 \times 10^{-2}$ & $0.123$ & $0.4712$ & $6.5$ & $6.3$ & $1.0$ & $0.5$ & $0.0$ & $0.8$ & $0.5$ & $-0.4$ & $0.0$ & $0.4$ & $0.0$ & $0.0$ \\ 
 
$500$ & $1.30 \times 10^{-1}$ & $0.076$ & $0.4112$ & $7.7$ & $7.5$ & $1.4$ & $0.6$ & $0.1$ & $1.2$ & $0.6$ & $-0.5$ & $0.0$ & $0.9$ & $0.0$ & $0.0$ \\ 
 
$500$ & $1.80 \times 10^{-1}$ & $0.055$ & $0.3045$ & $8.7$ & $8.4$ & $1.5$ & $0.6$ & $0.1$ & $1.4$ & $0.6$ & $-0.4$ & $-0.1$ & $1.1$ & $0.0$ & $0.0$ \\ 
 
$500$ & $2.50 \times 10^{-1}$ & $0.039$ & $0.2759$ & $8.5$ & $8.3$ & $1.9$ & $0.9$ & $0.8$ & $1.2$ & $0.9$ & $-0.6$ & $-0.2$ & $-0.3$ & $0.0$ & $0.0$ \\ 
 
$500$ & $4.00 \times 10^{-1}$ & $0.025$ & $0.1311$ & $13.7$ & $11.8$ & $4.1$ & $1.9$ & $3.1$ & $5.8$ & $1.8$ & $-0.7$ & $-0.7$ & $-5.3$ & $0.0$ & $0.0$ \\ 
 
$500$ & $6.50 \times 10^{-1}$ & $0.015$ & $0.01698$ & $27.9$ & $23.0$ & $7.0$ & $2.8$ & $5.9$ & $14.3$ & $2.8$ & $-1.4$ & $-1.0$ & $-13.9$ & $0.0$ & $0.0$ \\ 
 
\hline 
$650$ & $1.51 \times 10^{-2}$ & $0.850$ & $0.8058$ & $19.6$ & $19.4$ & $2.7$ & $0.5$ & $0.5$ & $1.1$ & $-0.1$ & $0.2$ & $0.1$ & $0.3$ & $0.7$ & $0.7$ \\ 
 
$650$ & $1.71 \times 10^{-2}$ & $0.750$ & $0.9192$ & $14.0$ & $13.9$ & $2.0$ & $0.1$ & $0.2$ & $0.4$ & $0.1$ & $-0.3$ & $0.0$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$650$ & $1.97 \times 10^{-2}$ & $0.650$ & $0.9125$ & $12.1$ & $12.0$ & $1.9$ & $0.0$ & $0.1$ & $0.4$ & $-0.1$ & $-0.4$ & $0.0$ & $0.1$ & $0.1$ & $0.0$ \\ 
 
$650$ & $2.61 \times 10^{-2}$ & $0.490$ & $0.6085$ & $8.0$ & $7.8$ & $1.8$ & $0.5$ & $0.0$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$650$ & $5.00 \times 10^{-2}$ & $0.256$ & $0.4952$ & $7.9$ & $7.8$ & $1.1$ & $0.6$ & $0.0$ & $0.8$ & $-0.6$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$650$ & $8.00 \times 10^{-2}$ & $0.160$ & $0.4515$ & $7.9$ & $7.8$ & $1.0$ & $0.4$ & $0.2$ & $0.8$ & $0.5$ & $-0.4$ & $0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$650$ & $1.30 \times 10^{-1}$ & $0.098$ & $0.3732$ & $9.5$ & $9.3$ & $1.4$ & $0.6$ & $0.2$ & $0.8$ & $0.6$ & $-0.4$ & $-0.1$ & $0.3$ & $0.0$ & $0.0$ \\ 
 
$650$ & $1.80 \times 10^{-1}$ & $0.071$ & $0.3397$ & $9.7$ & $9.5$ & $1.5$ & $0.5$ & $0.2$ & $1.1$ & $0.6$ & $-0.5$ & $0.0$ & $0.9$ & $0.0$ & $0.0$ \\ 
 
$650$ & $2.50 \times 10^{-1}$ & $0.051$ & $0.2520$ & $10.3$ & $10.1$ & $1.7$ & $0.7$ & $0.5$ & $0.9$ & $0.7$ & $-0.3$ & $0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$650$ & $4.00 \times 10^{-1}$ & $0.032$ & $0.1915$ & $12.8$ & $11.2$ & $3.9$ & $1.9$ & $2.7$ & $4.8$ & $1.9$ & $-0.8$ & $-0.7$ & $-4.3$ & $0.0$ & $0.0$ \\ 
 
$650$ & $6.50 \times 10^{-1}$ & $0.020$ & $0.02382$ & $27.6$ & $22.4$ & $7.8$ & $3.7$ & $6.4$ & $14.0$ & $3.5$ & $-1.1$ & $-1.2$ & $-13.5$ & $0.0$ & $0.0$ \\ 
 
\hline 
$800$ & $1.85 \times 10^{-2}$ & $0.850$ & $0.2872$ & $37.1$ & $36.9$ & $3.9$ & $1.1$ & $0.4$ & $0.5$ & $0.2$ & $-0.3$ & $0.0$ & $0.2$ & $0.3$ & $0.1$ \\ 
 
$800$ & $2.10 \times 10^{-2}$ & $0.750$ & $0.6634$ & $19.2$ & $19.0$ & $2.3$ & $0.2$ & $0.2$ & $0.3$ & $-0.1$ & $-0.2$ & $0.1$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$800$ & $2.42 \times 10^{-2}$ & $0.650$ & $0.6620$ & $16.0$ & $15.9$ & $2.1$ & $0.4$ & $0.1$ & $0.4$ & $-0.3$ & $-0.2$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$800$ & $3.21 \times 10^{-2}$ & $0.490$ & $0.6172$ & $8.8$ & $8.6$ & $1.8$ & $0.6$ & $0.0$ & $0.4$ & $-0.3$ & $-0.3$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$800$ & $5.00 \times 10^{-2}$ & $0.315$ & $0.4847$ & $9.1$ & $9.0$ & $1.2$ & $0.7$ & $0.0$ & $0.6$ & $-0.5$ & $-0.3$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$800$ & $8.00 \times 10^{-2}$ & $0.197$ & $0.4527$ & $9.3$ & $9.1$ & $1.3$ & $0.8$ & $0.0$ & $0.7$ & $-0.5$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$800$ & $1.30 \times 10^{-1}$ & $0.121$ & $0.3868$ & $10.8$ & $10.6$ & $1.4$ & $0.5$ & $0.3$ & $0.9$ & $0.7$ & $-0.4$ & $-0.2$ & $0.4$ & $0.0$ & $0.0$ \\ 
 
$800$ & $1.80 \times 10^{-1}$ & $0.087$ & $0.3642$ & $11.0$ & $10.9$ & $1.5$ & $0.2$ & $0.1$ & $0.8$ & $0.4$ & $-0.3$ & $0.0$ & $0.6$ & $0.0$ & $0.0$ \\ 
 
$800$ & $2.50 \times 10^{-1}$ & $0.063$ & $0.2749$ & $11.7$ & $11.6$ & $1.7$ & $0.6$ & $0.6$ & $1.0$ & $0.8$ & $-0.4$ & $-0.2$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$800$ & $4.00 \times 10^{-1}$ & $0.039$ & $0.1262$ & $16.7$ & $15.8$ & $3.5$ & $1.5$ & $2.3$ & $3.9$ & $1.5$ & $-0.4$ & $-0.6$ & $-3.5$ & $0.0$ & $0.0$ \\ 
 
$800$ & $6.50 \times 10^{-1}$ & $0.024$ & $0.01953$ & $31.8$ & $28.9$ & $7.1$ & $2.9$ & $5.9$ & $11.4$ & $2.8$ & $-0.7$ & $-1.0$ & $-11.0$ & $0.0$ & $0.0$ \\ 
 
\hline 
\end{tabular} 
\end{center} 
\caption{Continued from table~\ref{tab:xsec460}.} 
\end{table} 


==> plots/xsec575.tex <==
\begin{table}[htbp] 
\begin{center} 
\tiny 
\begin{tabular}{|r|c|c|r|r|r|r|r|r|r|r|r|r|r|r|r|} 
\hline 
$Q^2$ & $x$ & $y$ & $\tilde{\sigma}_{\rm NC}$ & 
$\delta_{\rm tot}$ & $\delta_{\rm stat}$ & $\delta_{\rm unc}$ & 
$\delta_{\rm unc}^{E}$ & 
$\delta_{\rm unc}^{h}$& 
$\delta_{\rm cor}$ & 
$\delta_{\rm cor}^{E^+}$ & 
$\delta_{\rm cor}^{\theta^+}$& 
$\delta_{\rm cor}^{h^+}$& 
$\delta_{\rm cor}^{N^+}$& 
$\delta_{\rm cor}^{S^+}$& 
$\delta_{\rm cor}^{D^+}$ \\ 
$(\rm GeV^2)$ & & & & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ 
\\ \hline 
$35$ & $6.50 \times 10^{-4}$ & $0.848$ & $1.303$ & $8.6$ & $7.1$ & $3.8$ & $0.5$ & $2.7$ & $3.1$ & $-0.2$ & $-0.5$ & $0.2$ & $0.6$ & $2.7$ & $1.2$ \\ 
 
\hline 
$45$ & $8.40 \times 10^{-4}$ & $0.848$ & $1.413$ & $7.2$ & $6.0$ & $3.4$ & $0.4$ & $2.2$ & $2.0$ & $-0.2$ & $-0.4$ & $0.1$ & $0.5$ & $1.6$ & $1.1$ \\ 
 
$45$ & $9.30 \times 10^{-4}$ & $0.760$ & $1.235$ & $8.2$ & $7.7$ & $2.6$ & $0.5$ & $0.7$ & $1.4$ & $-0.2$ & $-0.6$ & $0.1$ & $0.3$ & $0.7$ & $0.9$ \\ 
 
\hline 
$60$ & $1.11 \times 10^{-3}$ & $0.848$ & $1.259$ & $8.0$ & $7.1$ & $3.2$ & $0.3$ & $2.0$ & $1.8$ & $-0.1$ & $-0.4$ & $0.1$ & $0.5$ & $1.5$ & $0.8$ \\ 
 
$60$ & $1.24 \times 10^{-3}$ & $0.760$ & $1.411$ & $6.4$ & $5.8$ & $2.3$ & $0.7$ & $0.6$ & $1.3$ & $-0.4$ & $-0.5$ & $0.0$ & $0.2$ & $0.6$ & $1.0$ \\ 
 
$60$ & $1.39 \times 10^{-3}$ & $0.680$ & $1.268$ & $7.5$ & $7.2$ & $2.0$ & $0.5$ & $0.2$ & $1.1$ & $-0.2$ & $-0.6$ & $0.0$ & $0.2$ & $0.5$ & $0.7$ \\ 
 
\hline 
$90$ & $1.67 \times 10^{-3}$ & $0.848$ & $1.310$ & $8.6$ & $7.9$ & $2.9$ & $0.3$ & $1.7$ & $1.7$ & $-0.2$ & $-0.4$ & $0.1$ & $0.4$ & $1.4$ & $0.8$ \\ 
 
$90$ & $1.86 \times 10^{-3}$ & $0.760$ & $1.326$ & $6.9$ & $6.5$ & $2.1$ & $0.3$ & $0.5$ & $1.1$ & $-0.1$ & $-0.5$ & $0.0$ & $0.3$ & $0.3$ & $0.9$ \\ 
 
$90$ & $2.09 \times 10^{-3}$ & $0.680$ & $1.316$ & $6.2$ & $5.8$ & $1.9$ & $0.5$ & $0.2$ & $1.0$ & $-0.2$ & $-0.6$ & $0.0$ & $0.2$ & $0.2$ & $0.7$ \\ 
 
$90$ & $2.36 \times 10^{-3}$ & $0.600$ & $1.342$ & $6.4$ & $6.0$ & $2.0$ & $0.8$ & $0.1$ & $0.8$ & $-0.2$ & $-0.8$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
\hline 
$120$ & $2.23 \times 10^{-3}$ & $0.848$ & $1.374$ & $9.0$ & $8.4$ & $2.7$ & $0.3$ & $1.5$ & $1.4$ & $-0.2$ & $-0.4$ & $0.1$ & $0.4$ & $0.6$ & $1.1$ \\ 
 
$120$ & $2.49 \times 10^{-3}$ & $0.760$ & $1.173$ & $8.0$ & $7.7$ & $2.0$ & $0.6$ & $0.4$ & $0.8$ & $-0.3$ & $-0.3$ & $0.0$ & $0.2$ & $0.3$ & $0.6$ \\ 
 
$120$ & $2.78 \times 10^{-3}$ & $0.680$ & $1.161$ & $7.2$ & $6.9$ & $1.9$ & $0.4$ & $0.2$ & $0.6$ & $0.1$ & $-0.4$ & $0.0$ & $0.2$ & $0.2$ & $0.3$ \\ 
 
$120$ & $3.15 \times 10^{-3}$ & $0.600$ & $1.115$ & $6.8$ & $6.5$ & $1.8$ & $0.4$ & $0.1$ & $0.7$ & $-0.3$ & $-0.6$ & $0.0$ & $0.2$ & $0.3$ & $0.0$ \\ 
 
$120$ & $3.63 \times 10^{-3}$ & $0.520$ & $1.185$ & $6.0$ & $5.7$ & $1.8$ & $0.5$ & $0.1$ & $0.8$ & $-0.4$ & $-0.7$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$120$ & $4.82 \times 10^{-3}$ & $0.392$ & $1.074$ & $5.5$ & $5.1$ & $1.6$ & $0.5$ & $0.0$ & $1.0$ & $-0.3$ & $-0.9$ & $0.0$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
\hline 
$150$ & $2.79 \times 10^{-3}$ & $0.848$ & $1.291$ & $10.8$ & $10.3$ & $2.6$ & $0.3$ & $1.2$ & $1.8$ & $-0.1$ & $-0.3$ & $0.1$ & $0.4$ & $0.8$ & $1.5$ \\ 
 
$150$ & $3.11 \times 10^{-3}$ & $0.760$ & $1.171$ & $9.8$ & $9.5$ & $2.0$ & $0.3$ & $0.4$ & $1.0$ & $-0.2$ & $-0.5$ & $0.1$ & $0.3$ & $0.5$ & $0.6$ \\ 
 
$150$ & $3.47 \times 10^{-3}$ & $0.680$ & $1.324$ & $7.9$ & $7.6$ & $2.3$ & $1.3$ & $0.2$ & $0.6$ & $-0.1$ & $-0.5$ & $0.0$ & $0.2$ & $0.3$ & $0.2$ \\ 
 
$150$ & $3.94 \times 10^{-3}$ & $0.600$ & $1.244$ & $7.2$ & $6.9$ & $1.8$ & $0.2$ & $0.1$ & $0.6$ & $-0.2$ & $-0.5$ & $0.0$ & $0.1$ & $0.2$ & $0.0$ \\ 
 
$150$ & $4.54 \times 10^{-3}$ & $0.520$ & $1.041$ & $7.1$ & $6.8$ & $1.8$ & $0.3$ & $0.1$ & $0.7$ & $-0.3$ & $-0.6$ & $0.0$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$150$ & $6.03 \times 10^{-3}$ & $0.392$ & $1.020$ & $4.0$ & $3.6$ & $1.4$ & $0.7$ & $0.0$ & $0.8$ & $-0.5$ & $-0.6$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$150$ & $8.00 \times 10^{-3}$ & $0.295$ & $0.9700$ & $4.2$ & $3.9$ & $1.1$ & $0.8$ & $0.0$ & $0.9$ & $-0.5$ & $-0.8$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$150$ & $1.30 \times 10^{-2}$ & $0.182$ & $0.8609$ & $5.7$ & $5.2$ & $1.8$ & $1.4$ & $0.9$ & $1.2$ & $-0.9$ & $-0.6$ & $-0.2$ & $-0.5$ & $0.0$ & $0.0$ \\ 
 
$150$ & $2.00 \times 10^{-2}$ & $0.118$ & $0.7980$ & $7.8$ & $6.9$ & $2.8$ & $2.5$ & $1.0$ & $2.0$ & $-1.6$ & $-1.0$ & $-0.3$ & $-0.8$ & $0.0$ & $0.0$ \\ 
 
\hline 
$200$ & $3.72 \times 10^{-3}$ & $0.848$ & $1.296$ & $13.3$ & $12.9$ & $2.6$ & $0.1$ & $1.2$ & $2.0$ & $-0.2$ & $-0.3$ & $0.1$ & $0.3$ & $0.9$ & $1.7$ \\ 
 
$200$ & $4.15 \times 10^{-3}$ & $0.760$ & $1.288$ & $11.8$ & $11.5$ & $2.1$ & $0.2$ & $0.3$ & $1.2$ & $0.2$ & $-0.5$ & $0.0$ & $0.2$ & $0.1$ & $1.0$ \\ 
 
$200$ & $4.63 \times 10^{-3}$ & $0.680$ & $1.051$ & $11.3$ & $11.1$ & $2.2$ & $1.1$ & $0.2$ & $0.5$ & $0.2$ & $-0.3$ & $0.0$ & $0.2$ & $0.3$ & $0.2$ \\ 
 
$200$ & $5.25 \times 10^{-3}$ & $0.600$ & $1.169$ & $9.1$ & $8.9$ & $1.8$ & $0.2$ & $0.1$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$200$ & $6.06 \times 10^{-3}$ & $0.520$ & $1.110$ & $8.3$ & $8.1$ & $1.8$ & $0.2$ & $0.1$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$200$ & $8.04 \times 10^{-3}$ & $0.392$ & $0.9625$ & $4.8$ & $4.6$ & $1.3$ & $0.4$ & $0.0$ & $0.8$ & $-0.3$ & $-0.7$ & $0.0$ & $0.1$ & $0.1$ & $0.0$ \\ 
 
$200$ & $1.30 \times 10^{-2}$ & $0.242$ & $0.8743$ & $4.7$ & $4.4$ & $1.3$ & $1.0$ & $0.0$ & $1.0$ & $-0.6$ & $-0.7$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$200$ & $2.00 \times 10^{-2}$ & $0.157$ & $0.7573$ & $5.1$ & $4.9$ & $0.9$ & $0.3$ & $0.0$ & $0.8$ & $0.2$ & $-0.6$ & $-0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$200$ & $3.20 \times 10^{-2}$ & $0.098$ & $0.6151$ & $5.6$ & $5.5$ & $1.0$ & $0.5$ & $0.0$ & $0.6$ & $-0.3$ & $-0.5$ & $-0.1$ & $0.3$ & $0.0$ & $0.0$ \\ 
 
$200$ & $5.00 \times 10^{-2}$ & $0.063$ & $0.5041$ & $6.5$ & $6.4$ & $1.2$ & $0.6$ & $0.5$ & $0.8$ & $-0.4$ & $-0.6$ & $-0.2$ & $-0.1$ & $0.0$ & $0.0$ \\ 
 
$200$ & $8.00 \times 10^{-2}$ & $0.039$ & $0.4211$ & $7.7$ & $7.3$ & $1.7$ & $1.4$ & $0.2$ & $1.5$ & $-0.9$ & $-0.6$ & $-0.1$ & $1.1$ & $0.0$ & $0.0$ \\ 
 
$200$ & $1.30 \times 10^{-1}$ & $0.024$ & $0.3857$ & $7.6$ & $7.2$ & $1.9$ & $1.5$ & $0.2$ & $1.5$ & $-0.7$ & $-0.9$ & $-0.2$ & $0.9$ & $0.0$ & $0.0$ \\ 
 
$200$ & $1.80 \times 10^{-1}$ & $0.018$ & $0.3034$ & $10.4$ & $9.3$ & $2.6$ & $0.6$ & $2.1$ & $3.7$ & $-0.5$ & $-0.8$ & $-0.3$ & $-3.6$ & $0.0$ & $0.0$ \\ 
 
$200$ & $4.00 \times 10^{-1}$ & $0.008$ & $0.1910$ & $13.2$ & $11.0$ & $3.7$ & $0.7$ & $3.1$ & $6.3$ & $-0.5$ & $-1.2$ & $-0.4$ & $-6.1$ & $0.0$ & $0.0$ \\ 
 
\hline 
$250$ & $4.64 \times 10^{-3}$ & $0.848$ & $0.8545$ & $19.8$ & $19.5$ & $2.5$ & $0.2$ & $1.0$ & $2.5$ & $0.1$ & $-0.3$ & $0.1$ & $0.3$ & $1.4$ & $2.0$ \\ 
 
$250$ & $5.18 \times 10^{-3}$ & $0.760$ & $1.080$ & $14.3$ & $14.1$ & $2.2$ & $0.2$ & $0.3$ & $1.5$ & $0.1$ & $-0.4$ & $0.1$ & $0.2$ & $0.0$ & $1.4$ \\ 
 
$250$ & $5.79 \times 10^{-3}$ & $0.680$ & $0.9481$ & $13.9$ & $13.7$ & $2.3$ & $1.2$ & $0.1$ & $0.5$ & $-0.2$ & $-0.3$ & $0.0$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$250$ & $6.56 \times 10^{-3}$ & $0.600$ & $0.9475$ & $11.6$ & $11.5$ & $1.8$ & $0.2$ & $0.1$ & $0.5$ & $-0.1$ & $-0.4$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$250$ & $7.57 \times 10^{-3}$ & $0.520$ & $1.018$ & $9.8$ & $9.6$ & $1.8$ & $0.2$ & $0.1$ & $0.6$ & $-0.2$ & $-0.5$ & $0.0$ & $0.2$ & $0.1$ & $0.0$ \\ 
 
$250$ & $1.00 \times 10^{-2}$ & $0.392$ & $0.9523$ & $5.3$ & $5.1$ & $1.2$ & $0.4$ & $0.0$ & $0.6$ & $-0.3$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$250$ & $1.30 \times 10^{-2}$ & $0.303$ & $0.8513$ & $5.3$ & $5.1$ & $1.1$ & $0.6$ & $0.0$ & $0.8$ & $-0.6$ & $-0.5$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$250$ & $2.00 \times 10^{-2}$ & $0.197$ & $0.7707$ & $5.5$ & $5.2$ & $1.5$ & $1.2$ & $0.0$ & $1.1$ & $-0.9$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$250$ & $3.20 \times 10^{-2}$ & $0.123$ & $0.6210$ & $5.9$ & $5.7$ & $1.4$ & $1.0$ & $0.3$ & $1.0$ & $0.4$ & $-0.6$ & $0.0$ & $0.6$ & $0.0$ & $0.0$ \\ 
 
$250$ & $5.00 \times 10^{-2}$ & $0.079$ & $0.5412$ & $6.1$ & $5.9$ & $1.4$ & $1.0$ & $0.1$ & $0.9$ & $0.5$ & $-0.6$ & $0.0$ & $0.6$ & $0.0$ & $0.0$ \\ 
 
$250$ & $8.00 \times 10^{-2}$ & $0.049$ & $0.4602$ & $6.7$ & $6.4$ & $1.3$ & $0.9$ & $0.1$ & $1.3$ & $0.3$ & $-0.5$ & $-0.1$ & $1.2$ & $0.0$ & $0.0$ \\ 
 
$250$ & $1.30 \times 10^{-1}$ & $0.030$ & $0.3906$ & $6.6$ & $6.2$ & $1.4$ & $0.7$ & $0.2$ & $1.8$ & $0.3$ & $-0.5$ & $0.0$ & $1.8$ & $0.0$ & $0.0$ \\ 
 
$250$ & $1.80 \times 10^{-1}$ & $0.022$ & $0.3514$ & $7.8$ & $6.9$ & $2.5$ & $1.5$ & $1.5$ & $2.5$ & $0.7$ & $-0.6$ & $-0.4$ & $-2.3$ & $0.0$ & $0.0$ \\ 
 
$250$ & $4.00 \times 10^{-1}$ & $0.010$ & $0.1556$ & $13.0$ & $10.1$ & $4.2$ & $2.5$ & $2.7$ & $7.1$ & $1.5$ & $-1.0$ & $-0.5$ & $-6.8$ & $0.0$ & $0.0$ \\ 
 
\hline 
$300$ & $5.57 \times 10^{-3}$ & $0.848$ & $1.208$ & $16.0$ & $15.7$ & $2.5$ & $0.6$ & $0.8$ & $2.1$ & $-0.3$ & $-0.3$ & $0.1$ & $0.3$ & $0.2$ & $2.1$ \\ 
 
$300$ & $6.22 \times 10^{-3}$ & $0.760$ & $0.8707$ & $18.1$ & $18.0$ & $2.1$ & $0.2$ & $0.3$ & $1.3$ & $-0.2$ & $-0.4$ & $0.1$ & $0.2$ & $0.4$ & $1.1$ \\ 
 
$300$ & $6.95 \times 10^{-3}$ & $0.680$ & $0.9694$ & $15.0$ & $14.8$ & $2.1$ & $0.8$ & $0.1$ & $0.5$ & $-0.1$ & $-0.5$ & $0.0$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$300$ & $7.88 \times 10^{-3}$ & $0.600$ & $1.035$ & $12.9$ & $12.7$ & $1.9$ & $0.1$ & $0.1$ & $0.5$ & $0.1$ & $-0.5$ & $0.0$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$300$ & $9.09 \times 10^{-3}$ & $0.520$ & $0.8632$ & $12.1$ & $12.0$ & $1.8$ & $0.3$ & $0.1$ & $0.6$ & $-0.3$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$300$ & $1.21 \times 10^{-2}$ & $0.392$ & $0.9079$ & $6.2$ & $6.0$ & $1.3$ & $0.4$ & $0.0$ & $0.6$ & $-0.4$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$300$ & $2.00 \times 10^{-2}$ & $0.236$ & $0.6653$ & $6.5$ & $6.3$ & $1.0$ & $0.6$ & $0.0$ & $0.9$ & $-0.6$ & $-0.7$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$300$ & $3.20 \times 10^{-2}$ & $0.148$ & $0.6171$ & $6.7$ & $6.6$ & $1.0$ & $0.5$ & $0.1$ & $0.8$ & $0.3$ & $-0.4$ & $0.0$ & $0.6$ & $0.0$ & $0.0$ \\ 
 
$300$ & $5.00 \times 10^{-2}$ & $0.094$ & $0.5364$ & $6.9$ & $6.8$ & $1.2$ & $0.8$ & $0.0$ & $0.9$ & $0.5$ & $-0.6$ & $-0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$300$ & $8.00 \times 10^{-2}$ & $0.059$ & $0.4802$ & $7.4$ & $7.2$ & $1.3$ & $0.9$ & $0.0$ & $1.2$ & $0.5$ & $-0.6$ & $-0.1$ & $0.9$ & $0.0$ & $0.0$ \\ 
 
$300$ & $1.30 \times 10^{-1}$ & $0.036$ & $0.3762$ & $7.6$ & $7.2$ & $1.5$ & $1.0$ & $0.1$ & $1.9$ & $0.4$ & $-0.6$ & $-0.1$ & $1.7$ & $0.0$ & $0.0$ \\ 
 
$300$ & $1.80 \times 10^{-1}$ & $0.026$ & $0.3190$ & $8.7$ & $8.1$ & $2.5$ & $1.8$ & $1.1$ & $2.0$ & $1.1$ & $-0.9$ & $-0.3$ & $-1.4$ & $0.0$ & $0.0$ \\ 
 
$300$ & $4.00 \times 10^{-1}$ & $0.012$ & $0.1469$ & $15.5$ & $12.0$ & $4.8$ & $2.8$ & $3.4$ & $8.6$ & $1.7$ & $-1.1$ & $-0.6$ & $-8.4$ & $0.0$ & $0.0$ \\ 
 
\hline 

\end{tabular} 
\end{center} 
\caption[RESULT] 
{\sl \label{tab:xsec575} The NC 
$e^+p$ reduced cross section $\tilde{\sigma}_{\rm NC}(x,Q^2)$ 
for $E_p=575$ GeV and $P_e=0$ 
with statistical 
$(\delta_{\rm stat})$, 
total $(\delta_{tot})$, 
total uncorrelated systematic $(\delta_{\rm unc})$ 
errors, two of its contributions from the 
 electron energy error ($\delta_{unc}^{E}$)  
and the hadronic energy error  
($\delta_{\rm unc}^{h}$). 
The effect of the other uncorrelated 
systematic errors is included in $\delta_{\rm unc}$. 
In addition the correlated systematic  
$(\delta_{\rm cor})$ and its contributions from a 
positive variation of one  
standard deviation of the 
electron energy error ($\delta_{cor}^{E^+}$), of 
the polar electron angle error 
($\delta_{\rm cor}^{\theta^+}$), of the hadronic 
energy error ($\delta_{\rm cor}^{h^+}$), of the error 
due to noise subtraction ($\delta_{\rm cor}^{N^+}$), 
of the error 
due to background subtraction charge asymmetry 
 ($\delta_{\rm cor}^{S^+}$) 
and of the error 
due to variation of the cut value on the electron discriminator $D_{ele}$  
 ($\delta_{\rm cor}^{D^+}$) are given. 
The normalisation uncertainty is 
not included in the errors. 
The table continues on the next page.}
\end{table} 
\begin{table}[htbp] 
\begin{center} 
\tiny 
\begin{tabular}{|r|c|c|r|r|r|r|r|r|r|r|r|r|r|r|r|} 
\hline 
$Q^2$ & $x$ & $y$ & $\tilde{\sigma}_{\rm NC}$ & 
$\delta_{\rm tot}$ & $\delta_{\rm stat}$ & $\delta_{\rm unc}$ & 
$\delta_{\rm unc}^{E}$ & 
$\delta_{\rm unc}^{h}$& 
$\delta_{\rm cor}$ & 
$\delta_{\rm cor}^{E^+}$ & 
$\delta_{\rm cor}^{\theta^+}$& 
$\delta_{\rm cor}^{h^+}$& 
$\delta_{\rm cor}^{N^+}$& 
$\delta_{\rm cor}^{S^+}$& 
$\delta_{\rm cor}^{D^+}$ \\ 
$(\rm GeV^2)$ & & & & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & 
$(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ & $(\%)$ 
\\ \hline 
$400$ & $7.43 \times 10^{-3}$ & $0.848$ & $0.8123$ & $23.1$ & $22.9$ & $2.6$ & $0.3$ & $0.7$ & $2.3$ & $-0.3$ & $-0.3$ & $0.1$ & $0.3$ & $0.6$ & $2.2$ \\ 
 
$400$ & $8.29 \times 10^{-3}$ & $0.760$ & $0.5949$ & $23.1$ & $23.0$ & $2.3$ & $0.6$ & $0.2$ & $0.8$ & $-0.1$ & $-0.3$ & $0.0$ & $0.2$ & $0.0$ & $0.8$ \\ 
 
$400$ & $9.27 \times 10^{-3}$ & $0.680$ & $1.013$ & $16.1$ & $16.0$ & $2.0$ & $0.4$ & $0.2$ & $0.4$ & $0.2$ & $-0.2$ & $0.0$ & $0.2$ & $0.2$ & $0.0$ \\ 
 
$400$ & $1.05 \times 10^{-2}$ & $0.600$ & $0.8806$ & $15.6$ & $15.5$ & $1.9$ & $0.3$ & $0.1$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$400$ & $1.21 \times 10^{-2}$ & $0.520$ & $0.9991$ & $13.0$ & $12.9$ & $1.9$ & $0.1$ & $0.1$ & $0.5$ & $0.2$ & $-0.4$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$400$ & $1.61 \times 10^{-2}$ & $0.392$ & $0.8791$ & $7.1$ & $7.0$ & $1.2$ & $0.3$ & $0.0$ & $0.6$ & $-0.3$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$400$ & $3.20 \times 10^{-2}$ & $0.197$ & $0.6501$ & $7.3$ & $7.2$ & $1.1$ & $0.8$ & $0.0$ & $1.0$ & $-0.8$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$400$ & $5.00 \times 10^{-2}$ & $0.126$ & $0.5099$ & $8.0$ & $7.9$ & $1.1$ & $0.6$ & $0.1$ & $1.0$ & $0.6$ & $-0.6$ & $0.0$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$400$ & $8.00 \times 10^{-2}$ & $0.079$ & $0.4452$ & $8.6$ & $8.5$ & $1.1$ & $0.6$ & $0.1$ & $1.1$ & $0.6$ & $-0.6$ & $-0.1$ & $0.7$ & $0.0$ & $0.0$ \\ 
 
$400$ & $1.30 \times 10^{-1}$ & $0.049$ & $0.3769$ & $8.5$ & $8.2$ & $1.3$ & $0.4$ & $0.2$ & $1.7$ & $0.4$ & $-0.4$ & $0.0$ & $1.6$ & $0.0$ & $0.0$ \\ 
 
$400$ & $1.80 \times 10^{-1}$ & $0.035$ & $0.3421$ & $8.9$ & $8.6$ & $2.0$ & $1.0$ & $1.1$ & $1.6$ & $0.9$ & $-0.6$ & $-0.3$ & $-1.1$ & $0.0$ & $0.0$ \\ 
 
$400$ & $4.00 \times 10^{-1}$ & $0.016$ & $0.1488$ & $16.6$ & $13.4$ & $4.6$ & $2.0$ & $3.5$ & $8.6$ & $1.9$ & $-0.9$ & $-0.7$ & $-8.4$ & $0.0$ & $0.0$ \\ 
 
\hline 
$500$ & $9.29 \times 10^{-3}$ & $0.848$ & $0.7285$ & $27.8$ & $27.6$ & $2.7$ & $0.3$ & $0.5$ & $2.1$ & $0.0$ & $-0.1$ & $0.1$ & $0.2$ & $0.4$ & $2.1$ \\ 
 
$500$ & $1.04 \times 10^{-2}$ & $0.760$ & $0.7348$ & $22.8$ & $22.7$ & $2.3$ & $1.0$ & $0.3$ & $0.5$ & $-0.2$ & $-0.4$ & $0.1$ & $0.2$ & $0.0$ & $0.1$ \\ 
 
$500$ & $1.16 \times 10^{-2}$ & $0.680$ & $1.177$ & $16.2$ & $16.1$ & $2.0$ & $0.1$ & $0.1$ & $0.4$ & $-0.1$ & $-0.3$ & $0.0$ & $0.2$ & $0.0$ & $0.0$ \\ 
 
$500$ & $1.31 \times 10^{-2}$ & $0.600$ & $0.8538$ & $17.7$ & $17.6$ & $1.9$ & $0.2$ & $0.1$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.1$ & $0.2$ & $0.0$ \\ 
 
$500$ & $1.51 \times 10^{-2}$ & $0.520$ & $1.040$ & $14.2$ & $14.1$ & $1.9$ & $0.4$ & $0.1$ & $0.4$ & $-0.3$ & $-0.3$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$500$ & $2.01 \times 10^{-2}$ & $0.392$ & $0.7340$ & $9.1$ & $9.0$ & $1.3$ & $0.4$ & $0.0$ & $0.6$ & $-0.4$ & $-0.4$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$500$ & $3.20 \times 10^{-2}$ & $0.246$ & $0.6891$ & $8.4$ & $8.3$ & $1.1$ & $0.7$ & $0.0$ & $0.8$ & $-0.7$ & $-0.4$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$500$ & $5.00 \times 10^{-2}$ & $0.157$ & $0.5602$ & $8.9$ & $8.8$ & $1.0$ & $0.3$ & $0.4$ & $0.8$ & $0.3$ & $-0.3$ & $0.1$ & $0.7$ & $0.0$ & $0.0$ \\ 
 
$500$ & $8.00 \times 10^{-2}$ & $0.098$ & $0.4454$ & $9.8$ & $9.7$ & $1.0$ & $0.5$ & $0.2$ & $0.7$ & $0.5$ & $-0.3$ & $-0.1$ & $0.3$ & $0.0$ & $0.0$ \\ 
 
$500$ & $1.30 \times 10^{-1}$ & $0.061$ & $0.3831$ & $11.5$ & $11.4$ & $1.3$ & $0.5$ & $0.2$ & $1.4$ & $0.5$ & $-0.4$ & $0.1$ & $1.3$ & $0.0$ & $0.0$ \\ 
 
$500$ & $1.80 \times 10^{-1}$ & $0.044$ & $0.3467$ & $11.6$ & $11.3$ & $1.5$ & $0.6$ & $0.1$ & $1.6$ & $0.6$ & $-0.5$ & $-0.1$ & $1.4$ & $0.0$ & $0.0$ \\ 
 
$500$ & $2.50 \times 10^{-1}$ & $0.032$ & $0.2290$ & $13.8$ & $13.5$ & $2.0$ & $0.8$ & $1.2$ & $1.7$ & $0.8$ & $-0.4$ & $-0.3$ & $-1.4$ & $0.0$ & $0.0$ \\ 
 
$500$ & $4.00 \times 10^{-1}$ & $0.020$ & $0.1687$ & $18.1$ & $16.3$ & $4.2$ & $1.8$ & $3.2$ & $6.7$ & $1.8$ & $-0.6$ & $-0.7$ & $-6.3$ & $0.0$ & $0.0$ \\ 
 
$500$ & $6.50 \times 10^{-1}$ & $0.012$ & $0.02022$ & $31.5$ & $28.9$ & $5.5$ & $2.3$ & $4.3$ & $11.2$ & $2.3$ & $-0.9$ & $-0.7$ & $-10.9$ & $0.0$ & $0.0$ \\ 
 
\hline 
$650$ & $1.21 \times 10^{-2}$ & $0.848$ & $0.4914$ & $38.7$ & $38.5$ & $3.0$ & $0.4$ & $0.4$ & $1.0$ & $0.2$ & $0.0$ & $0.0$ & $0.2$ & $0.5$ & $0.8$ \\ 
 
$650$ & $1.35 \times 10^{-2}$ & $0.760$ & $0.6986$ & $28.3$ & $28.2$ & $2.2$ & $0.3$ & $0.2$ & $0.6$ & $-0.2$ & $-0.2$ & $0.1$ & $0.2$ & $0.4$ & $0.0$ \\ 
 
$650$ & $1.51 \times 10^{-2}$ & $0.680$ & $0.6789$ & $25.2$ & $25.1$ & $2.1$ & $0.2$ & $0.1$ & $0.5$ & $0.1$ & $-0.3$ & $0.0$ & $0.2$ & $0.3$ & $0.0$ \\ 
 
$650$ & $1.71 \times 10^{-2}$ & $0.600$ & $0.6957$ & $21.4$ & $21.3$ & $2.0$ & $0.3$ & $0.1$ & $0.5$ & $-0.2$ & $-0.4$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$650$ & $1.97 \times 10^{-2}$ & $0.520$ & $0.4817$ & $22.7$ & $22.6$ & $2.0$ & $0.6$ & $0.1$ & $0.6$ & $-0.4$ & $-0.4$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$650$ & $2.61 \times 10^{-2}$ & $0.392$ & $0.6348$ & $10.8$ & $10.7$ & $1.3$ & $0.4$ & $0.0$ & $0.5$ & $-0.2$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$650$ & $5.00 \times 10^{-2}$ & $0.205$ & $0.4685$ & $11.7$ & $11.6$ & $1.3$ & $0.9$ & $0.0$ & $1.0$ & $-0.8$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$650$ & $8.00 \times 10^{-2}$ & $0.128$ & $0.4525$ & $11.4$ & $11.3$ & $1.1$ & $0.5$ & $0.0$ & $0.9$ & $0.6$ & $-0.4$ & $-0.1$ & $0.5$ & $0.0$ & $0.0$ \\ 
 
$650$ & $1.30 \times 10^{-1}$ & $0.079$ & $0.3975$ & $13.4$ & $13.3$ & $1.4$ & $0.6$ & $0.0$ & $1.2$ & $0.6$ & $-0.5$ & $0.0$ & $0.9$ & $0.0$ & $0.0$ \\ 
 
$650$ & $1.80 \times 10^{-1}$ & $0.057$ & $0.3285$ & $14.0$ & $13.9$ & $1.4$ & $0.3$ & $0.2$ & $1.4$ & $0.4$ & $-0.2$ & $0.0$ & $1.4$ & $0.0$ & $0.0$ \\ 
 
$650$ & $2.50 \times 10^{-1}$ & $0.041$ & $0.2401$ & $15.5$ & $15.3$ & $2.0$ & $1.0$ & $0.9$ & $1.3$ & $1.0$ & $-0.6$ & $-0.3$ & $-0.6$ & $0.0$ & $0.0$ \\ 
 
$650$ & $4.00 \times 10^{-1}$ & $0.026$ & $0.1563$ & $20.4$ & $18.9$ & $4.5$ & $2.1$ & $3.3$ & $6.2$ & $2.2$ & $-0.9$ & $-0.9$ & $-5.7$ & $0.0$ & $0.0$ \\ 
 
$650$ & $6.50 \times 10^{-1}$ & $0.016$ & $0.02266$ & $35.8$ & $33.3$ & $6.0$ & $2.3$ & $4.9$ & $11.4$ & $2.2$ & $-0.9$ & $-0.8$ & $-11.1$ & $0.0$ & $0.0$ \\ 
 
\hline 
$800$ & $1.49 \times 10^{-2}$ & $0.848$ & $0.6679$ & $31.9$ & $31.8$ & $3.1$ & $0.9$ & $0.4$ & $0.5$ & $-0.4$ & $-0.2$ & $0.1$ & $0.2$ & $0.0$ & $0.1$ \\ 
 
$800$ & $1.66 \times 10^{-2}$ & $0.760$ & $0.4843$ & $38.5$ & $38.4$ & $2.7$ & $0.6$ & $0.2$ & $0.7$ & $0.6$ & $-0.3$ & $0.1$ & $0.3$ & $0.0$ & $0.0$ \\ 
 
$800$ & $1.85 \times 10^{-2}$ & $0.680$ & $0.6761$ & $27.1$ & $27.0$ & $2.2$ & $0.2$ & $0.1$ & $0.4$ & $-0.2$ & $-0.3$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$800$ & $2.10 \times 10^{-2}$ & $0.600$ & $0.6604$ & $24.5$ & $24.4$ & $2.1$ & $0.1$ & $0.1$ & $0.5$ & $-0.1$ & $-0.5$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$800$ & $2.42 \times 10^{-2}$ & $0.520$ & $0.6435$ & $21.9$ & $21.8$ & $1.9$ & $0.1$ & $0.0$ & $0.6$ & $0.0$ & $-0.6$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$800$ & $3.21 \times 10^{-2}$ & $0.392$ & $0.4923$ & $13.6$ & $13.5$ & $1.4$ & $0.5$ & $0.0$ & $0.4$ & $-0.3$ & $-0.3$ & $0.0$ & $0.1$ & $0.0$ & $0.0$ \\ 
 
$800$ & $5.00 \times 10^{-2}$ & $0.252$ & $0.5837$ & $12.0$ & $11.9$ & $1.2$ & $0.7$ & $0.0$ & $0.8$ & $-0.6$ & $-0.6$ & $0.0$ & $0.0$ & $0.0$ & $0.0$ \\ 
 
$800$ & $8.00 \times 10^{-2}$ & $0.157$ & $0.5522$ & $12.0$ & $12.0$ & $1.1$ & $0.4$ & $0.1$ & $0.8$ & $0.6$ & $-0.4$ & $0.1$ & $0.3$ & $0.0$ & $0.0$ \\ 
 
$800$ & $1.30 \times 10^{-1}$ & $0.097$ & $0.2926$ & $18.3$ & $18.3$ & $1.3$ & $0.1$ & $0.1$ & $0.7$ & $0.4$ & $-0.2$ & $-0.1$ & $0.6$ & $0.0$ & $0.0$ \\ 
 
$800$ & $1.80 \times 10^{-1}$ & $0.070$ & $0.2636$ & $18.7$ & $18.6$ & $1.5$ & $0.5$ & $0.1$ & $1.5$ & $0.7$ & $-0.5$ & $0.0$ & $1.2$ & $0.0$ & $0.0$ \\ 
 
$800$ & $2.50 \times 10^{-1}$ & $0.050$ & $0.1811$ & $20.5$ & $20.4$ & $1.9$ & $0.8$ & $0.8$ & $1.3$ & $1.1$ & $-0.5$ & $-0.2$ & $-0.5$ & $0.0$ & $0.0$ \\ 
 
$800$ & $4.00 \times 10^{-1}$ & $0.032$ & $0.1614$ & $22.2$ & $21.3$ & $3.8$ & $1.5$ & $2.7$ & $4.9$ & $1.5$ & $-0.4$ & $-0.5$ & $-4.6$ & $0.0$ & $0.0$ \\ 
 
$800$ & $6.50 \times 10^{-1}$ & $0.019$ & $0.02134$ & $43.1$ & $40.8$ & $6.7$ & $2.6$ & $5.4$ & $12.1$ & $2.7$ & $-0.6$ & $-1.1$ & $-11.8$ & $0.0$ & $0.0$ \\ 
 
\hline 
\end{tabular} 
\end{center} 
\caption{\label{tab:xsec575b} Continued from table~\ref{tab:xsec575}.} 
\end{table} 

